REGAS: REspiratory-GAted Synthesis of Views for Multi-Phase CBCT Reconstruction from a single 3D CBCT Acquisition

It is a long-standing challenge to reconstruct Cone Beam Computed Tomography (CBCT) of the lung under respiratory motion. This work takes a step further to address a challenging setting in reconstructing a multi-phase}4D lung image from just a single}3D CBCT acquisition. To this end, we introduce REpiratory-GAted Synthesis of views, or REGAS. REGAS proposes a self-supervised method to synthesize the undersampled tomographic views and mitigate aliasing artifacts in reconstructed images. This method allows a much better estimation of between-phase Deformation Vector Fields (DVFs), which are used to enhance reconstruction quality from direct observations without synthesis. To address the large memory cost of deep neural networks on high resolution 4D data, REGAS introduces a novel Ray Path Transformation (RPT) that allows for distributed, differentiable forward projections. REGAS require no additional measurements like prior scans, air-flow volume, or breathing velocity. Our extensive experiments show that REGAS significantly outperforms comparable methods in quantitative metrics and visual quality.

==> AAAI2023 REGAS (3)/RPT.tex <==
\subsection{Ray Path Transformation (RPT)}

Processing 4D CBCT data with a reasonable resolution limits the possible capacity of CNNs due to computational constraints. One way to mitigate this limitation is to reduce the input size via patch processing. Assuming the emitted rays traverse in Cartesian planes (e.g., in Parallel-Beam or Fan-Beam CT), one can separate the observed volume into slices~[\citeauthor{pmid32575088}], therefore dramatically reduces the input size. However, it is less straightforward to perform such a separation under a Cone-Beam imaging geometry, as rays traverse multiple Cartesian planes. Motivated by the fact that a tomographic view only partially observes the desired volume during CBCT acquisition, we instead seek to reduce computation by including only the observed volume when synthesizing a tomographic view.


To this end, REGAS implements a Ray Path Transformation (RPT) operator $\mathcal{T}$. Given a view angle $a_k$, RPT transforms a CBCT volume from a Cartesian-based representation $V\in \mathbb{R}^{X\times Y\times Z}$ to view-based representation $R_{a_k}\in \mathbb{R}^{W\times H\times S}$, such that $P(a_k, w, h) = \sum_{s=1}^SR_{a_k}(w, h, s)$, where $S$ is the marching dimension of each ray, and $P(a_k) \in \mathbb{R}^{W\times H}$ is the tomographic view under angle $a_k$. Mathematically, the RPT operator $\mathcal{T}$ can be described as:
\begin{align}\label{eqn: RPT}
\begin{aligned}
    \mathcal{T}(V, a_k) = R_{a_k}, R_{a_k}(w,h,s) = V( \bm{l}^{a_k}_{w,h}(s)),
\end{aligned}
\end{align}
where $\bm{l}^{a_k}_{w,h}$ denotes the line segment that connects point $(w,h)$ in $P(a_k)$ and the ray source. As such, $R_{a_k}(w,h,s)$ is the minimum representation of $V$ to produce $P(a_k)$, and can be split and recombined over the $w-h$ plane while maintaining integrity to the Cone Beam forward projection geometry, as demonstrated in Fig.~\ref{fig:network}. This property enables patch training and for REGAS and scales REGAS to synthesize high resolution views. RPT is implemented through CUDA with gradient propagation, and is as fast as other GPU-based forward projection operations.

==> AAAI2023 REGAS (3)/abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
It is a long-standing challenge to reconstruct Cone Beam Computed Tomography (CBCT) of the lung under respiratory motion. This work takes a step further to address a challenging setting in reconstructing a \textbf{multi-phase} 4D lung image from just a \textbf{single} 3D CBCT acquisition.
% with minimum constraints.
To this end, we introduce \underline{RE}piratory-\underline{GA}ted \underline{S}ynthesis of views, or \textbf{REGAS}. REGAS proposes a self-supervised method to synthesize the undersampled tomographic views and mitigate aliasing artifacts in reconstructed images. This method allows a much better estimation of between-phase Deformation Vector Fields (DVFs), which are used to enhance reconstruction quality from direct observations \textit{without synthesis}. To address the large memory cost of deep neural networks on high resolution 4D data, REGAS introduces a novel Ray Path Transformation (RPT) that allows for \textit{distributed, differentiable} forward projections. REGAS require no additional measurements like prior scans, air-flow volume, or breathing velocity. Our extensive experiments show that REGAS significantly outperforms comparable methods in quantitative metrics and visual quality.


% It is a long-standing challenge to reconstruct Cone Beam Computed Tomography (CBCT) of the lung under respiratory motion. This work takes a step further to address an even more challenging setting where we aim to reconstruct a multi-phase 4D lung image from just a single 3D CBCT acquisition. To this end, we introduce REpiratory-GAted Synthesis of views, or REGAS. REGAS proposes a self-supervised method to synthesize the undersampled tomographic views and mitigate the aliasing artifacts in reconstructed images. This also enables a better estimation of between-phase Deformation Vector Fields (DVFs), which can then be used to further enhance reconstruction quality. Moreover, to address the training of deep neural networks on high resolution 4D data, REGAS introduces a novel Ray Path Transformation (RPT) that allows for distributed, differentiable forward projections. REGAS require no additional measurements like prior scans, air-flow volume, or breathing velocity. Our extensive experiments show that REGAS significantly outperforms comparable methods in terms of quantitative metrics and visual quality.
\end{abstract}

==> AAAI2023 REGAS (3)/conclusion.tex <==
% \vspace{-0.7em}
\section{Conclusion}

We propose REGAS, a novel 4D CBCT reconstruction method from a single 3D CBCT acquisition. On a high level, REGAS first formulates sparse-view phase reconstruction as a synthesis problem on unobserved views. By combining observed and synthesized views, REGAS can obtain reconstructions with significantly less artifacts. REGAS then finds inter-phase DVFs based on these reconstructions, and use a synthesis-free optimization to refine reconstructions based on DVFs and observed views. Within REGAS, we propose RPT, which transforms a CT volume into a ray-based representation. The RPT-transformed volumes can be separated for distributed, patch-based training without affecting the Cone Beam imaging geometry, which addresses the memory bottleneck during network training. REGAS' network is trained in a self-supervised manner and does not require groundtruth on unobserved views, and is practical for clinical application. Our evaluation on a 4D Lung dataset show that REGAS significantly outperforms comparable methods in reconstruction performance. REGAS can assist in more accurate CBCT-based image-guided radiation therapy with high quality reconstructions. Since RPT reduces the memory footprint of 3D volume in a DL-based 3D-to-2D hybrid system, it can be applied to tasks that benefit from fusion learning on 3D CT and 2D radiographs, e.g. landmark detection, lesion segmentation, without sacrificing resolution.

==> AAAI2023 REGAS (3)/experiments.tex <==
\section{Experiments}
\textbf{Dataset.} Evaluating the effectiveness of respiratory-gated CBCT reconstruction on real acquisition data has some major challenges: 1. there is no gold-standard groundtruth for unobserved views of a phase due to constant breathing motion; 2. CBCT images are acquired with low dosage and tend to be noisy; 3. due to the enormous file sizes of 4D acquisition data, public dataset for respiratory-gated CBCT is scarce and only from very few patients, e.g. five cases in SPARE \cite{shieh2019spare} on the Varian system. As a proof-of-concept, we use the 4D Lung dataset from Hugo et. al.\cite{2017A}, which contains 62 high quality ten-phased 4D FBCTs, to perform experiments based on realistic simulations. Specifically, we synthesize $P_{i,a_k}$ as Digitally Reconstructed Radiographs (DRRs) \cite{milickovic2000ct} by using the projection geometry from real respiratory-gated acquisitions in SPARE. We set detector size to $\{W=256,H=192\}$, detector spacing to $1.55mm$, and the total number of acquired views to $K=680$. CT volumes are normalized to an isotropic resolution of $1.5mm$ and a resolution of $128\times256\times256$. The phase-view correspondences $\phi(*)$ are from real measurements in SPARE after aligning the max-inhale and max-exhale phases with \cite{2017A}. We use OSSART to obtain $V^{\textrm{init}}_{i}$. For RPT, the ray marching dimension is set to $S=128$; during training $R^{\textrm{init}}_{i,a_k}$ are separated into patches of $128\times128\times128$. 

%This FBCT-simulated setup also allows us to study the effectiveness of CNN-based transfer learning for RG-CBCT reconstruction without a significant domain gap. We use the LIDC-IDRI dataset[], which contains 890 lung FBCT volumes after pre-processing, to simulate the low quality reconstructions due to irregular sparse-view sampling in RG-CBCT.

% \subsection{Implementation Details}
% REGAS is trained end-to-end. For 3D CNN, REGAS uses a 3D-UNet \cite{DBLP:conf/miccai/RonnebergerFB15} structure, where five downsampling and upsampling CNN layers are used. A 2D Residual DenseNet (RDN \cite{DBLP:conf/cvpr/ZhangTKZ018}) is used for the projection-refining stage, where we use ten residual dense blocks, each of which has six convolution layers and growing rate of thirty-two. We use the ANTs package for DVF estimation, specifically by using cross correlation as the regression loss. We use TIGRE for OSSART reconstruction. We train all the models with Adam
% optimization, with a momentum of 0.5 and a learning rate of 0.0001, until they converge. For more about model architectures, please refer to the Supplemental Material. 

\input{imgs/recon_imgs}
\textbf{Baselines.} We examine the effectiveness of RPT and each component within the network structure by experimenting alternative implementations, including:

\begin{itemize}
\item $\textrm{REGAS}_{\textrm{2D}}$: We remove $\mathcal{G}$ of REGAS, and use only $\mathcal{F}$ to improve the quality of unseen views directly from $V^{\textrm{init}}_{i}$; we use losses described in Eq. (\ref{eqn: recon_loss}) and (\ref{eqn: 2DCNN_GAN}).
\item $\textrm{REGAS}_{\textrm{noMA}}$: We use REGAS without the motion averaging loss in Eq. (\ref{eqn:3D_loss}).
\item $\textrm{REGAS}_{\textrm{noRPT}}$: We use REGAS without RPT, i.e. providing $V^{\textrm{init}}_{i}$ as inputs to $\mathcal{G}$ and perform forward projection on the output volume; we then use $\mathcal{F}$ to improve synthesized view quality. $V^{\textrm{init}}_{i}$ is bicubically downsampled to $128\times128\times128$ due to memory constraint. 
% \item $\textrm{REGAS}_{DVF}$: We use REGAS with the DVF-based post-processing described in section \ref{sec:dvf}.
\end{itemize}


 We also study the effectiveness of the mainstream DL-based sparse-view reconstruction approaches, which use CNNs to recover artifact-free images from the sparse-view affected reconstructions through supervised learning. As we use 4D FBCTs for simulation and testing, we can use a CNN to train on an external FBCT dataset without suffering from a large domain gap during testing. Note that this is a \emph{theoretical} exercise; in reality it is extremely difficult to obtain artifact free, high quality CBCT groundtruth in large scale. LIDC-IDRI \cite{armato2011lung}, which contains 890 FBCT lung images after pre-processing, is used to simulate sparse-view reconstructions for training data. For fair comparison, we use 3D-UNet \cite{DBLP:conf/miccai/CicekALBR16} as the network architecture, and an $\mathcal{L}_{1}$ reconstruction loss for training. We denote such a baseline as $\textrm{UNet}_{\textrm{sup}}$. Quantitatively, we use Peak Signal-to-Noise Ratio (PSNR) and Structural SIMilarity (SSIM) \cite{DBLP:journals/tip/WangBSS04} to measure performance. Additional discussions about data processing, simulation, and other implementation details are available in the supplemental material section.
 
 
 
%  $\textrm{UNet}_{\textrm{sup}}$ follows the general approaches of [][][], which recover artifact-free images from the sparse-view affected inputs by using a CNN learned through supervision. As our experiments are performed on simulated data on FBCTs, it allows us to study the effectiveness of $\textrm{UNet}_{\textrm{sup}}$ for RG-CBCT reconstruction without a significant domain gap. For fair comparison, we use $\mathcal{G}$ in REGAS as the network for $\textrm{UNet}_{\textrm{sup}}$, and train it on the simulated data based on the LIDC-IDRI dataset. The simulation is performed according to that of 4D FBCTs used for inference and described in section \ref{sec:data}. 
% note that $K_{7}=40$, thus phase 7 is severely undersampled
% \input{imgs/projs}

% \input{imgs/dvf_imgs}
\subsection{Quantitative Evaluation}
We summarize the performance of different reconstruction approaches in Table \ref{tab:sota_table} and visualize the results in Fig. \ref{tab:ablation_img} over different phases. As we can see, due to limited and irregular sparse-view sampling, artifacts are quite severe in OSSART. In particular, we observe that some bone structural details are completely lost in phase 7. 
Due to severe sparse-view artifacts, $\textrm{UNet}_{\textrm{sup}}$ cannot recover these details in the reconstructed image domain. In fact, $\textrm{UNet}_{\textrm{sup}}$ generally oversmoothes the inputs due to training with $\mathcal{L}_{1}$ loss; consequently, even bone details that are observable through OSSART are lost in reconstructions by $\textrm{UNet}_{\textrm{sup}}$. We also observe that $\textrm{UNet}_{\textrm{sup}}$ can mistake sparse-view artifacts for real tissues and produce unfaithful details. As such, $\textrm{UNet}_{\textrm{sup}}$ is clinically unreliable despite its relatively high performance in PSNR. $\textrm{REGAS}_{\textrm{2D}}$ directly applies the 2D part of REGAS on views from $V^{\textrm{init}}_{i}$; however, these views can be very blurry due to undersampled reconstruction. Therefore, it is difficult for networks to recover views that are consistent with the underlying geometry. While $\textrm{REGAS}_{\textrm{noRPT}}$ performs slightly better than $\textrm{REGAS}_{\textrm{2D}}$ both quantitatively and visually, its information loss due to downsampling in 3D leads to lost details in 2D views and requires $\mathcal{F}$ to recover them via GAN. $\textrm{REGAS}_{\textrm{noMA}}$ shows good performance compared to the other two ablated methods, but does not share patterns as well as the full REGAS in 3D due to the lack of $\mathcal{L}_{\textrm{MA}}$. We show an instance of the synthesized views in Fig \ref{fig:proj} for all versions of REGAS. In particular, we can see that views from $\textrm{REGAS}_{\textrm{noRPT}}$ and $\textrm{REGAS}_{\textrm{noMA}}$ both recover the rib cage frame on the right side of the lung. Compared to the full REGAS, there is less clarity over the heart region in $\textrm{REGAS}_{\textrm{noMA}}$ due to the noisier 3D CTs, and $\textrm{REGAS}_{\textrm{noRPT}}$ generates more fictitious details. The full REGAS produces a much more stable and geometrically consistent synthesis, thus demonstrating the utility of each component and the effectiveness of scaling computation complexity with distributed forward projections. Please refer to the supplemental material on how volumetric resolution impacts views visually and other intermediate results.

Ideally, the synthesized views should be reintroduced to the 4D reconstruction space and updated, which helps reduce geometric inconsistencies; however, such a step is infeasible due to computing limitations. Since the 4D reconstruction space is too large to be addressed at a voxel level, DVF-based reconstruction provides an alternative solution that is less sensitive to per-voxel accuracy. 
\subsection{Deformed FBP Reconstruction}\label{sec:dvf_exp}
We apply the DVF-based post-processing described in section \ref{sec:dvf} on REGAS-reconstructed $V^{\textrm{VS}}_{i}$ to obtain $V^{\textrm{DVF}}_{i}$ through SyN \cite{AVANTS200826}. Similar post-processing can be applied to OSSART and ${\textrm{UNet}}_{\textrm{sup}}$, where we replace $V^{\textrm{VS}}_{i}$ with their respective reconstructions to find between-phase DVFs. These methods are denoted as $\textrm{REGAS}^{\textrm{DVF}}$, $\textrm{OSSART}^{\textrm{DVF}}$, and $\textrm{UNet}^{\textrm{DVF}}_{\textrm{sup}}$. Quantitative measurements are shown in Table \ref{tab:sota_table}, and visualizations are shown in Fig. \ref{tab:dvf_img}.  
Clearly, using real views for reconstruction eliminates a significant amount of streaking artifacts from the inaccuracies in synthesized views. However, artifacts induced by erroneous DVFs exist. By using bones as static markers, we can observe that results from $\textrm{OSSART}^{\textrm{DVF}}$ deform randomly from phase to phase due to unreliable DVFs, as indicated by the orange arrows. Such deformations are also observable in $\textrm{UNet}^{\textrm{DVF}}_{\textrm{sup}}$ to a lesser extent, as shown in the blurry spine reconstruction. In particular, as $\textrm{UNet}_{\textrm{sup}}$ tends to blur out details, the estimated DVFs can globally drift in the direction of the motion, as indicated by the yellow arrow in Fig. \ref{tab:dvf_img}.
In comparison, $\textrm{REGAS}^{\textrm{DVF}}$ estimates more accurate DVFs and produces higher definition reconstructions, where deformations only happen to motion-affected area.




% despite high PSNR measurements. As results from REGAS are of much higher quality, $\textrm{REGAS}^{\textrm{DVF}}$ is more stable. 

% use bones as static markers and find they shift significantly from phase to phase in results from $\textrm{OSSART}^{\textrm{DVF}}$ and, to a smaller degree, from $\textrm{UNet}^{\textrm{DVF}}_{\textrm{sup}}$, as indicated by the orange arrows in Fig. \ref{tab:dvf_img}. 
We note that minor drifts of otherwise static structures, e.g. the bones, are hard to be completely avoided for DVF-based reconstruction, as the estimated DVFs will be imperfect in describing the breathing motion even from groundtruth phases. In comparison, reconstructions from the vanilla REGAS do not suffer from this problem as convolutions do not produce geometric changes on synthesized views. Despite lower PSNR metrics, the vanilla REGAS may be preferable over $\textrm{REGAS}^{\textrm{DVF}}$ in certain scenarios. Please refer to the supplemental material for animated results of $\textrm{OSSART}^{\textrm{DVF}}$ and $\textrm{REGAS}^{\textrm{DVF}}$.

REGAS can be incorporated into iterative DVF-based methods, such as SMEIR \cite{wang2013simultaneous} and MC-SART \cite{chee2019mcsart}, in place of SART as the initial DVF-based reconstruction. As REGAS significantly reduces noise in reconstructed CBCTs, iterative DVF-based methods can benefit from fewer iterations and higher likelihood of convergence. Furthermore, it is likely that an iterative version of REGAS, where $V^{\textrm{init}}_{i}$ are replaced with reconstructed $V^{\textrm{VS}}_{i}$ from a previous iteration, can further enhance performance. REGAS also has a potential advantage in its application on real CBCT acquisition; specifically, traditional methods that derive from ART-based reconstructions use DRR to generate views, thus they suffer from a significant domain gap as DRR does not simulate real projections well \cite{DBLP:journals/corr/abs-2012-02407,DBLP:conf/miccai/UnberathZLBFAN18}. In comparison, REGAS has a view-refining CNN $\mathcal{F}$ that is GAN-based, and should help reduce such domain gaps. We plan to apply REGAS on real CBCT acquisitions in a future study.




%Note that this is different from methods such as SMEIR in a few ways: 1. there is no iteration as we can immediately obtain high quality DVFs; however, it is feasible that incorporation of iterative methods like SMEIR can help us find better DVFs; 2. reconstruction is done by warping each projection to every phase. In methods like SMEIR, due to computational complexity and issues in convergence, only $\mathcal{M}_{0\rightarrow j}$ are calculated. As the estimated DVFs likely cannot perfectly describe the transitions between phases, we find a larger number of DVF estimations leads to more accurate reconstructions.


% $\textrm{REGAS}_{\textrm{noRPT}}$, and REGAS, denoted as $\textrm{OSSART}^{\textrm{DVF}}$, $\textrm{REGAS}^{\textrm{DVF}}_{\textrm{noRPT}}$, and $\textrm{REGAS}^{\textrm{DVF}}$.

==> AAAI2023 REGAS (3)/experiments_new.tex <==
\section{Experiments}
\textbf{Dataset.} To quantitatively evaluate the effectiveness of respiratory-gated CBCT reconstruction, we follow previous works~\cite{wang2013simultaneous,pmid32575088,chee2019mcsart} in simulating the acquisition process based on Digitally Reconstructed Radiographs (DRRs)~\cite{milickovic2000ct}. Specifically, we use the 4D Lung dataset~\cite{2017A}, which contains 62 high quality ten-phased 4D Fan-Beam CTs, and the projection geometry from real respiratory-gated acquisitions~\cite{shieh2019spare}. We set detector size to $\{W=256,H=192\}$, detector spacing to $1.55mm$, and the total number of acquired views to $K=680$. CT volumes are normalized to an isotropic resolution of $1.5mm$ and a resolution of $128\times256\times256$. While REGAS can be scaled to higher resolutions than $P \in \mathbb{R}^{256\times 192}$ and $V \in \mathbb{R}^{128\times 256\times 256}$, these resolutions are selected to ensure that other comparative methods stay computationally feasible in memory and time. The phase-view correspondences are based on real measurements in~\cite{shieh2019spare} after aligning the max-inhale and max-exhale phases with~\cite{2017A}. We use OSSART to obtain $V^{\textrm{init}}_{i}$. For RPT, the ray marching dimension is set to $S=128$; during training $R^{\textrm{init}}_{i,a_k}$ are separated into patches of $128\times128\times128$. While our REGAS method is self-supervised, thus requiring no training data, the comparative DL-based supervised methods (U-Net and DL-PICCS) are trained on LIDC-IDRI~\cite{armato2011lung}, which contains 890 FBCT lung images after pre-processing. The same data generation method is used to obtain the undersampled reconstructions as inputs, where for each image three random phases and their respective $P^{obs}_i$ are selected.



\subsection{Implementation Details}

The VSN in REGAS is trained end-to-end with an Adam optimizer, which uses a momentum of 0.5 and a learning rate of 0.0001 until convergence. For 3D CNN, REGAS uses a 3D-UNet \cite{DBLP:conf/miccai/RonnebergerFB15} structure, where five downsampling and upsampling CNN layers are used. A 2D Residual DenseNet (RDN \cite{DBLP:conf/cvpr/ZhangTKZ018}) is used for the view-refining stage, where we use ten residual dense blocks, each of which has six convolution layers and growing rate of thirty-two. We use 10 NVIDIA 2080TI to train the network in one day. While patch training is used due to the memory cost of backpropagation, at inference time $P^{\textrm{syn}}$ are generated with full resolution. It takes 28.75ms to synthesize one view, or 176s to synthesize all views for one 4D CBCT image on a single NVIDIA 2080TI. We use VoxelMorph~\cite{DBLP:journals/tmi/BalakrishnanZSG19} for DVF estimation, where all $V^{\textrm{syn}}_i$ are used for training. We use 6 NVIDIA 2080TI GPUs to train VoxelMorph for one day to obtain the desired model. This is similarly done for all methods that use inter-phase modelling, i.e. $\textrm{SMEIR}^{\textrm{sim}}$ and DVF-GT. We use TIGRE\footnote{https://github.com/CERN/TIGRE} for OSSART reconstruction. Please see the supplemental material section for more details. %We also perform ablation study on REGAS by removing RPT, $\mathcal{L}_{\textrm{MA}}$, or  $\mathcal{L}_{\textrm{GAN}}$ from the formulation. 
\input{imgs/recon_imgs}
% \textbf{Baselines.} We examine the effectiveness of RPT and each component within the network structure by experimenting alternative implementations, including:

% \begin{itemize}
% \item $\textrm{REGAS}_{\textrm{2D}}$: We remove $\mathcal{G}$ of REGAS, and use only $\mathcal{F}$ to improve the quality of unseen views directly from $V^{\textrm{init}}_{i}$; we use losses described in Eq. (\ref{eqn: recon_loss}) and (\ref{eqn: 2DCNN_GAN}).
% \item $\textrm{REGAS}_{\textrm{noMA}}$: We use REGAS without the motion averaging loss in Eq. (\ref{eqn:3D_loss}).
% \item $\textrm{REGAS}_{\textrm{noRPT}}$: We use REGAS without RPT, i.e. providing $V^{\textrm{init}}_{i}$ as inputs to $\mathcal{G}$ and perform forward projection on the output volume; we then use $\mathcal{F}$ to improve synthesized view quality. $V^{\textrm{init}}_{i}$ is bicubically downsampled to $128\times128\times128$ due to memory constraint. 
% % \item $\textrm{REGAS}_{DVF}$: We use REGAS with the DVF-based post-processing described in section \ref{sec:dvf}.
% \end{itemize}


%  We also study the effectiveness of the mainstream DL-based sparse-view reconstruction approaches, which use CNNs to recover artifact-free images from the sparse-view affected reconstructions through supervised learning. As we use 4D FBCTs for simulation and testing, we can use a CNN to train on an external FBCT dataset without suffering from a large domain gap during testing. Note that this is a \emph{theoretical} exercise; in reality it is extremely difficult to obtain artifact free, high quality CBCT groundtruth in large scale. LIDC-IDRI \cite{armato2011lung}, which contains 890 FBCT lung images after pre-processing, is used to simulate sparse-view reconstructions for training data. For fair comparison, we use 3D-UNet \cite{DBLP:conf/miccai/CicekALBR16} as the network architecture, and an $\mathcal{L}_{1}$ reconstruction loss for training. We denote such a baseline as $\textrm{UNet}_{\textrm{sup}}$. Quantitatively, we use Peak Signal-to-Noise Ratio (PSNR) and Structural SIMilarity (SSIM) \cite{DBLP:journals/tip/WangBSS04} to measure performance. Additional discussions about data processing, simulation, and other implementation details are available in the supplemental material section.
 
 
\subsection{Quantitative Evaluations}
We summarize the quantitative comparisons of different reconstruction approaches against REGAS in Table \ref{tab:sota_table}. These approaches include:

\begin{itemize}
\item OSSART~\cite{andersen1984simultaneous}: A classic algebraic sparse-view reconstruction method; spatial TV is used to ensure smoothness in reconstructed images.
\item $\textrm{OSSART}^{\textrm{TTV}}$: OSSART with an additional Temporal TV term during reconstruction optimization, similar to~\cite{Ritschl_2012}.
\item U-Net: A supervised DL method based on the 3D U-Net architecture, representative of end-to-end approaches like~\cite{DBLP:journals/tmi/HanY18}.
\item DL-PICCS~\cite{https://doi.org/10.1002/mp.15183}: A multi-staged supervised DL method that applies PICCS between stages.
\item $\textrm{SMEIR}^{\textrm{sim}}$: A DVF-based optimization method based on~\cite{wang2013simultaneous}, where the DVFs are estimated from OSSART reconstructions.
\item DVF-GT: An upper-bound analysis on the DVF-based refinement approach, where the DVFs are obtained from groundtruth images. 
\end{itemize}

We visualize the results in Fig. \ref{tab:quant_img} over different phases. As we can see for OSSART, due to motion-induced irregular sampling, aliasing artifacts vary in phases 1 and 8, which have 105 and 50 $P^{\textrm{obs}}_i$ respectively. Details like rib bones are difficult to distinguish in phase 8, and clearer in phase 1. For clarity, we divide the rest of the baselines based on whether they model inter-phase information or not. 

\textbf{Single-phase-only modelling approaches.} Here we mainly focus on DL-based methods, as they are the current state of the art in sparse-view CT reconstruction without inter-phase modelling. The U-Net approach, which operates purely in the image space, clearly suffers from over-smoothing, especially in phase 8, as the pixel-wise loss leads to averaging when artifact is severe. This is somewhat improved in DL-PICCS, which contains two U-Nets. The results from the first U-Net are updated with $P^{\textrm{obs}}_i$ in an OSSART manner, which recovers some lost details that can be observed in OSSART. Despite such an update, the bone details are still not fully recovered in phase 8. 

We note that there are DL-based methods that attempt to leverage the temporal information, such as 4D-AirNet~\cite{pmid32575088}. However, 4D-AirNet is constrained to work on 2D slices instead of the native 3D space for Cone Beam geometry, as the GPU memory cost would be infeasible if the network is updated with 3D kernels. As such, it is restricted to Fan Beam geometry if view consistency is to be enforced. 

While DL-PICCS is chosen as a representative baseline, as it has a step to ensure view consistency like 4D-AirNet and is trained in two stages to avoid memory constraints; we note that DL-PICCS uses all memory in a NVIDIA 2080Ti GPU with a batch size of one.
Compute feasibility is an important factor in DL-based methods, and is a strength of REGAS. REGAS addresses the undersampling problem by synthesizing views instead of directly operating in the higher-dimension image space. With RPT, REGAS can be trained in patches while preserving CBCT geometry; this greatly scales its ability to use deeper networks while still generating high quality views. 
While RPT is used for reconstruction in REGAS, its functions to obtain minimum 3D representation with respect to a view and to propagate gradients are generally useful, such as for any DL-based method that looks to leverage CT and X-ray images together for learning. Finally, REGAS is self-supervised, and can avoid domain gaps such as scanner or patient differences from a training set. While $P^{\textrm{syn}}_i$ are not perfect and still lead to some artifacts, as in Fig.~\ref{tab:quant_img} for  $\textrm{REGAS}^{\textrm{noDVF}}$, bone details are much better recovered. 

\textbf{Inter-phase modelling approaches.} Here, the dominant approaches are non-DL-based approaches, which are less reliant on GPU memory and leverage the temporal correlations between phases. A common approach is to add a Temporal TV term during the reconstruction optimization process, as represented by $\textrm{OSSART}^{\textrm{TTV}}$. While $\textrm{OSSART}^{\textrm{TTV}}$ greatly out-performs OSSART in PSNR, its superior performance is based on the fact that the phase voxels are mostly stationary with each other; however, details remain blurry due to movements, as such errors around the edges are very high. 

SMEIR focuses on finding the optimal DVFs between phases from limited acquisition, such that we can reconstruct phases with $P^{\textrm{obs}}$ as described in Eq.~(\ref{eqn:dvf_refine}). Specifically, it finds DVFs through an iterative scheme, where (\romannumeral 1) DVFs are first estimated from initial SART reconstructions, (\romannumeral 2) a reference phase is updated following Eq.~(\ref{eqn:dvf_refine}), and (\romannumeral 3) DVFs are updated based on observed views from other phases and the reference phase. Steps 2 and 3 are repeated to obtain better reference phase and DVFs. SMEIR contains many hyper-parameters for its iterative optimization process, and does not have a public implementation for reference. Furthermore, as stated by the authors, the DVFs are not guaranteed to converge. To avoid an unfaithful re-implementation, we simplify SMEIR to steps 1 and 2 with no iteration, referred to as $\textrm{SMEIR}^{\textrm{sim}}$. $\textrm{SMEIR}^{\textrm{sim}}$ is comparable to REGAS since both involve a reconstruction step and a DVF-based refinement step. Similarly, both should benefit from iterative updates if they converge. We observe that due to the superior reconstructions of REGAS from synthesized views, the DVFs are estimated with more accuracy and lead to high quality reconstructions. The artifacts from $\textrm{REGAS}^{\textrm{noDVF}}$ are gone, as only real acquisitions are used. In comparison, while the $\textrm{SMEIR}^{\textrm{sim}}$ results are seemingly alias-free, the erroneous DVFs lead to inconsistent deformations around the body surface, which can be observed in the phase 8 difference image in Fig.~\ref{tab:quant_img}. 



\textbf{Upper-bound analysis.} We also perform an upper-bound analysis called DVF-GT, where the DVFs are estimated directly from groundtruth phases and used in Eq.~(\ref{eqn:dvf_refine}). Since there does not exist a perfect DVF that leads to lossless phase reconstruction, DVF-GT represents the upper bounds of the DVF-based refinement step. We find that REGAS approaches DVF-GT in performance, particularly in SSIM  where REGAS is on par with DVF-GT. As such, we believe that REGAS approaches the upper limit from DVF-based refinement. 


\input{imgs/projs}

\input{tables/ablation}


\textbf{Ablation study.} We examine the effective of individual components in REGAS. $\textrm{REGAS}^{\textrm{2D}}$ trains the 2D CNN $\mathcal{F}$ with $\mathcal{L}_{\textrm{rec}}$ and $\mathcal{L}_{\textrm{GAN}}$ by directly using projections from $V^{\textrm{init}}_i$. With a 3D CNN $\mathcal{G}$, $\textrm{REGAS}^{\textrm{noRPT}}$ does not use RPT and has to downsample $V^{\textrm{init}}_i$ to $\mathbb{R}^{128\times 128\times 128}$ to be memory-wise viable. $\textrm{REGAS}^{\textrm{noMA}}$ does not use $\mathcal{L}_{\textrm{MA}}$, which denoises in 3D. As we can see in Table~\ref{tab:ablation}, adding $\mathcal{G}$, RPT, and $\mathcal{L}_{\textrm{MA}}$ each has a positive effect on performance. We show an instance of the synthesized views in Fig. \ref{fig:proj} for all versions of REGAS. In particular, we can see that views from $\textrm{REGAS}^{\textrm{noRPT}}$ and $\textrm{REGAS}^{\textrm{noMA}}$ both recover the rib cage frame on the right side of the lung. Compared to the full REGAS, there is less clarity over the heart region in $\textrm{REGAS}^{\textrm{noMA}}$ due to the noisier 3D CTs, and $\textrm{REGAS}^{\textrm{noRPT}}$ generates more fictitious details. The full REGAS produces a much more stable and geometrically consistent synthesis by leveraging DVF estimations from $\textrm{REGAS}^{\textrm{noRPT}}$ and real observations, which do not contain synthetic details. As such, we demonstrate the utility of each component and the effectiveness of scaling computation complexity with distributed forward projections. Please refer to the supplemental material on how volumetric resolution impacts views visually and other intermediate results.

% Please see the supplemental material section for more details on the effect of each component; animated visualizations of all compared methods are also provided.

% \vspace{-0.5em}

% \subsection{Limitations}
% While REGAS demonstrates excellent performances, it is based on DRRs. Performance on real 4D CBCT acquisition is difficult to be evaluated quantitatively, as there exists neither a large public dataset nor reliable groundtruth in real acquisitions. As a proof of concept study, REGAS follows all the mentioned baselines in its usage of simulated acquisitions. We note that the adversarial loss can be adopted to synthesize realistic CBCT views acquired under various settings, and will perform future study on clinical data. %Lastly, the self-supervised VSN is trained and evaluated on all 62 4D CTs due to the small sample size; given a larger dataset, a test set can be separated to better examine the performance of REGAS on unseen acquisitions. We expect REGAS to gain better performance with a larger dataset and accelerated reconstruction speed, similar to VoxelMorph~\cite{DBLP:journals/tmi/BalakrishnanZSG19}, and leave this for future study.




% Due to severe sparse-view artifacts, $\textrm{UNet}_{\textrm{sup}}$ cannot recover these details in the reconstructed image domain. In fact, $\textrm{UNet}_{\textrm{sup}}$ generally oversmoothes the inputs due to training with $\mathcal{L}_{1}$ loss; consequently, even bone details that are observable through OSSART are lost in reconstructions by $\textrm{UNet}_{\textrm{sup}}$. We also observe that $\textrm{UNet}_{\textrm{sup}}$ can mistake sparse-view artifacts for real tissues and produce unfaithful details. As such, $\textrm{UNet}_{\textrm{sup}}$ is clinically unreliable despite its relatively high performance in PSNR. $\textrm{REGAS}_{\textrm{2D}}$ directly applies the 2D part of REGAS on views from $V^{\textrm{init}}_{i}$; however, these views can be very blurry due to undersampled reconstruction. Therefore, it is difficult for networks to recover views that are consistent with the underlying geometry. While $\textrm{REGAS}_{\textrm{noRPT}}$ performs slightly better than $\textrm{REGAS}_{\textrm{2D}}$ both quantitatively and visually, its information loss due to downsampling in 3D leads to lost details in 2D views and requires $\mathcal{F}$ to recover them via GAN. $\textrm{REGAS}_{\textrm{noMA}}$ shows good performance compared to the other two ablated methods, but does not share patterns as well as the full REGAS in 3D due to the lack of $\mathcal{L}_{\textrm{MA}}$. We show an instance of the synthesized views in Fig \ref{fig:proj} for all versions of REGAS. In particular, we can see that views from $\textrm{REGAS}_{\textrm{noRPT}}$ and $\textrm{REGAS}_{\textrm{noMA}}$ both recover the rib cage frame on the right side of the lung. Compared to the full REGAS, there is less clarity over the heart region in $\textrm{REGAS}_{\textrm{noMA}}$ due to the noisier 3D CTs, and $\textrm{REGAS}_{\textrm{noRPT}}$ generates more fictitious details. The full REGAS produces a much more stable and geometrically consistent synthesis, thus demonstrating the utility of each component and the effectiveness of scaling computation complexity with distributed forward projections. Please refer to the supplemental material on how volumetric resolution impacts views visually and other intermediate results.

% Ideally, the synthesized views should be reintroduced to the 4D reconstruction space and updated, which helps reduce geometric inconsistencies; however, such a step is infeasible due to computing limitations. Since the 4D reconstruction space is too large to be addressed at a voxel level, DVF-based reconstruction provides an alternative solution that is less sensitive to per-voxel accuracy. 
% \subsection{Deformed FBP Reconstruction}\label{sec:dvf_exp}
% We apply the DVF-based post-processing described in section \ref{sec:dvf} on REGAS-reconstructed $V^{\textrm{VS}}_{i}$ to obtain $V^{\textrm{DVF}}_{i}$ through SyN \cite{AVANTS200826}. Similar post-processing can be applied to OSSART and ${\textrm{UNet}}_{\textrm{sup}}$, where we replace $V^{\textrm{VS}}_{i}$ with their respective reconstructions to find between-phase DVFs. These methods are denoted as $\textrm{REGAS}^{\textrm{DVF}}$, $\textrm{OSSART}^{\textrm{DVF}}$, and $\textrm{UNet}^{\textrm{DVF}}_{\textrm{sup}}$. Quantitative measurements are shown in Table \ref{tab:sota_table}, and visualizations are shown in Fig. \ref{tab:dvf_img}.  
% Clearly, using real views for reconstruction eliminates a significant amount of streaking artifacts from the inaccuracies in synthesized views. However, artifacts induced by erroneous DVFs exist. By using bones as static markers, we can observe that results from $\textrm{OSSART}^{\textrm{DVF}}$ deform randomly from phase to phase due to unreliable DVFs, as indicated by the orange arrows. Such deformations are also observable in $\textrm{UNet}^{\textrm{DVF}}_{\textrm{sup}}$ to a lesser extent, as shown in the blurry spine reconstruction. In particular, as $\textrm{UNet}_{\textrm{sup}}$ tends to blur out details, the estimated DVFs can globally drift in the direction of the motion, as indicated by the yellow arrow in Fig. \ref{tab:dvf_img}.
% In comparison, $\textrm{REGAS}^{\textrm{DVF}}$ estimates more accurate DVFs and produces higher definition reconstructions, where deformations only happen to motion-affected area.



% We note that minor drifts of otherwise static structures, e.g. the bones, are hard to be completely avoided for DVF-based reconstruction, as the estimated DVFs will be imperfect in describing the breathing motion even from groundtruth phases. In comparison, reconstructions from the vanilla REGAS do not suffer from this problem as convolutions do not produce geometric changes on synthesized views. Despite lower PSNR metrics, the vanilla REGAS may be preferable over $\textrm{REGAS}^{\textrm{DVF}}$ in certain scenarios. Please refer to the supplemental material for animated results of $\textrm{OSSART}^{\textrm{DVF}}$ and $\textrm{REGAS}^{\textrm{DVF}}$.

% REGAS can be incorporated into iterative DVF-based methods, such as SMEIR \cite{wang2013simultaneous} and MC-SART \cite{chee2019mcsart}, in place of SART as the initial DVF-based reconstruction. As REGAS significantly reduces noise in reconstructed CBCTs, iterative DVF-based methods can benefit from fewer iterations and higher likelihood of convergence. Furthermore, it is likely that an iterative version of REGAS, where $V^{\textrm{init}}_{i}$ are replaced with reconstructed $V^{\textrm{VS}}_{i}$ from a previous iteration, can further enhance performance. REGAS also has a potential advantage in its application on real CBCT acquisition; specifically, traditional methods that derive from ART-based reconstructions use DRR to generate views, thus they suffer from a significant domain gap as DRR does not simulate real projections well \cite{DBLP:journals/corr/abs-2012-02407,DBLP:conf/miccai/UnberathZLBFAN18}. In comparison, REGAS has a view-refining CNN $\mathcal{F}$ that is GAN-based, and should help reduce such domain gaps. We plan to apply REGAS on real CBCT acquisitions in a future study.




%Note that this is different from methods such as SMEIR in a few ways: 1. there is no iteration as we can immediately obtain high quality DVFs; however, it is feasible that incorporation of iterative methods like SMEIR can help us find better DVFs; 2. reconstruction is done by warping each projection to every phase. In methods like SMEIR, due to computational complexity and issues in convergence, only $\mathcal{M}_{0\rightarrow j}$ are calculated. As the estimated DVFs likely cannot perfectly describe the transitions between phases, we find a larger number of DVF estimations leads to more accurate reconstructions.


% $\textrm{REGAS}_{\textrm{noRPT}}$, and REGAS, denoted as $\textrm{OSSART}^{\textrm{DVF}}$, $\textrm{REGAS}^{\textrm{DVF}}_{\textrm{noRPT}}$, and $\textrm{REGAS}^{\textrm{DVF}}$.

==> AAAI2023 REGAS (3)/imgs/dvf_imgs.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{|ccccc|}
        \hline
        Phase & $\textrm{OSSART}^{\textrm{DVF}}$& $\textrm{UNet}^{\textrm{DVF}}_{\textrm{sup}}$&$\textrm{REGAS}^{\textrm{DVF}}$ & $\textrm{GT}$\\
        %&$\textrm{OSSART}^{DVF}_{sag}$&$\textrm{RG-Syn}^{DVF}_{sag}$ & $\textrm{GT}_{sag}$\\
        
        % -6$\degree$ & -3$\degree$ & 0$\degree$ (Input View) & 3$\degree$ & 6$\degree$ & 9$\degree$  \\
        2 & 
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ossart_cor_1_arrow.png}
            \caption{\hspace{4em}38.62/0.970}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ossart_sag_1.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/sup_cor_1.png}
            \caption{\hspace{4em}40.27/0.977}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/sup_sag_1.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ours_cor_1.png}
            \caption{\hspace{4em}\bf{41.79/0.982}}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ours_sag_1.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&        
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/gt_cor_1.png}
            \caption{\hspace{4em}PSNR/SSIM}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/gt_sag_1.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}\\
        
        7 & 
        
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ossart_cor_6_arrow.png}
            \caption{\hspace{4em}35.09/0.983}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ossart_sag_6.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/sup_cor_6_arrow.png}
            \caption{\hspace{4em}36.33/0.970}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/sup_sag_6_arrow.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ours_cor_6.png}
            \caption{\hspace{4em}\bf{40.89/0.982}}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ours_sag_6.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&        
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/gt_cor_6.png}
            \caption{\hspace{4em}PSNR/SSIM}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/gt_sag_6.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}\\        
        
        9 & 
        
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ossart_cor_8_arrow.png}
            \caption{\hspace{4em}36.91/0.962}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ossart_sag_8.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/sup_cor_8.png}
            \caption{\hspace{4em}39.69/0.976}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/sup_sag_8_arrow.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ours_cor_8.png}
            \caption{\hspace{4em}\bf{41.16/0.980}}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ours_sag_8.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&        
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/gt_cor_8.png}
            \caption{\hspace{4em}PSNR/SSIM}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/gt_sag_8.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}\\     
        \hline
    \end{tabular}
    \caption{Visual comparisons of DVF-based reconstructions. Static structures as indicated by the orange arrows shift significantly in $\textrm{OSSART}^{\textrm{DVF}}$ due to badly estimated DVFs. Metrics are calculated volume-wise.}
    \label{tab:dvf_img}
    \vspace{-1.5em}
\end{figure*}

==> AAAI2023 REGAS (3)/imgs/intro.tex <==
\begin{figure}[!tb]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{2pt}
    \vspace{-1em}
    \begin{tabular}[b]{cc}
        \multicolumn{2}{c}{
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\textwidth]{imgs/Intro.PNG}
            \caption{CBCT acquisitions}
            \label{CBCT_acq}
        \end{subfigure}
        } \\
        \begin{subfigure}[b]{.245\linewidth}
            \includegraphics[width=\textwidth]{imgs/FBP_recon.png}
            \caption{FDK}
            \label{FBP}
        \end{subfigure} &
        \begin{subfigure}[b]{.755\linewidth}
            \includegraphics[width=\textwidth]{imgs/RGPS_recon.png}
            \caption{Ours, shown in phase 1, 3, and 5}
            \label{RGPS}
        \end{subfigure} \\
    \end{tabular}
    \caption{The respiratory motion leads to inconsistencies between projections, thus the traditionally reconstructed image, \textit{e.g.} in \ref{FBP}, contains significant motion blur. Our proposed REGAS can disentangle the observed motion, as indicated by the orange arrows in \ref{RGPS}.}
    \label{fig:intro}
    \vspace{-1.5em}
\end{figure}

%As shown in \ref{CBCT_acq}, CBCT acquires X-ray projections of the body over different angles and reconstructs them in 3D. 

==> AAAI2023 REGAS (3)/imgs/proj_res.tex <==

\begin{figure}[!htb]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}[b]{cc}
        \begin{subfigure}[b]{.5\linewidth}
            \includegraphics[width=\textwidth]{imgs/proj_res/proj128.png}
            \caption{$\textrm{P}^{\textrm{LR}}$}
        \end{subfigure} &
        \begin{subfigure}[b]{.5\linewidth}
            \includegraphics[width=\textwidth]{imgs/proj_res/proj256.png}
            \caption{$\textrm{P}^{\textrm{HR}}$}
        \end{subfigure} \\
    \end{tabular}
    \caption{A visual comparison of forward projection quality. $P^{\textrm{HR}}$ and $P^{\textrm{LR}}$ are obtained from $V^{\textrm{HR}}\in \mathbb{R}^{128\times256\times256}$ and $V^{\textrm{LR}}\in \mathbb{R}^{128\times128\times128}$. The blue arrows indicate area where the bone details are lost in $P^{\textrm{LR}}$. }
    \label{fig:proj_res}
\end{figure}

==> AAAI2023 REGAS (3)/imgs/projs.tex <==
\begin{figure}[!htb]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}[b]{cc}
        \begin{subfigure}[b]{.5\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs/2d.png}
            \caption{$\textrm{REGAS}^{\textrm{2D}}$}
        \end{subfigure} &
        \begin{subfigure}[b]{.5\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs/orig.png}
            \caption{$\textrm{REGAS}^{\textrm{noRPT}}$}
        \end{subfigure} \\
        \begin{subfigure}[b]{.5\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs/noMA.png}
            \caption{$\textrm{REGAS}^{\textrm{noMA}}$}
        \end{subfigure} &
        \begin{subfigure}[b]{.5\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs/ours.png}
            \caption{$\textrm{REGAS}^{\textrm{noDVF}}$}
        \end{subfigure} \\
    \end{tabular}
    \caption{Visual Comparison of synthesized projections over various ablated methods, taken from phase 7.}
    \label{fig:proj}
\end{figure}

==> AAAI2023 REGAS (3)/imgs/projs_regas.tex <==

\begin{figure}[!htb]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}[b]{ccc}
        \begin{subfigure}[b]{.33\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs_regas/phase1_init.png}
            \caption{$\textrm{P}^{\textrm{init}}_{1,a_k}$}
        \end{subfigure} &
        \begin{subfigure}[b]{.33\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs_regas/phase1_ref.png}
            \caption{$\textrm{P}^{\textrm{ref}}_{1,a_k}$}
        \end{subfigure} &
        \begin{subfigure}[b]{.33\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs_regas/phase1_out.png}
            \caption{$\textrm{P}^{\textrm{syn}}_{1,a_k}$}
        \end{subfigure} \\
        \begin{subfigure}[b]{.33\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs_regas/phase2_init.png}
            \caption{$\textrm{P}^{\textrm{init}}_{2,a_k}$}
        \end{subfigure} &
        \begin{subfigure}[b]{.33\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs_regas/phase2_ref.png}
            \caption{$\textrm{P}^{\textrm{ref}}_{2,a_k}$}
        \end{subfigure} &
        \begin{subfigure}[b]{.33\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs_regas/phase2_out.png}
            \caption{$\textrm{P}^{\textrm{syn}}_{2,a_k}$}
        \end{subfigure} \\
        \begin{subfigure}[b]{.33\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs_regas/phase3_init.png}
            \caption{$\textrm{P}^{\textrm{init}}_{3,a_k}$}
        \end{subfigure} &
        \begin{subfigure}[b]{.33\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs_regas/phase3_ref.png}
            \caption{$\textrm{P}^{\textrm{ref}}_{3,a_k}$}
        \end{subfigure} &
        \begin{subfigure}[b]{.33\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs_regas/phase3_out.png}
            \caption{$\textrm{P}^{\textrm{syn}}_{3,a_k}$}
        \end{subfigure} \\
    \end{tabular}
    
    \begin{tabular}[b]{cc}
        \hspace{3.5em}
        \begin{subfigure}[b]{.33\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs_regas/phase1_gt.png}
            \caption{$\textrm{P}^{\textrm{obs}}_{1,a_k}$}
        \end{subfigure} &
        \begin{subfigure}[b]{.33\linewidth}
            \includegraphics[width=\textwidth]{imgs/projs_regas/proj_ma.png}
            \caption{$\textrm{P}^{\textrm{ma}}_{a_k}$}
        \end{subfigure} \\
    \end{tabular}
    \caption{REGAS's intermediate results for phases $i=\{1,2,3\}$ are visualized as projections from view angle $a_k$. $\textrm{P}^{\textrm{init}}_{i,a_k}$,$\textrm{P}^{\textrm{ref}}_{i,a_k}$, and $\textrm{P}^{\textrm{syn}}_{i,a_k}$ are projections from the initial OSSART reconstructions, after going through $\mathcal{G}$, and after going through $\mathcal{F}$. The observed projection $\textrm{P}^{\textrm{obs}}_{1,a_k}$ and projection from $V^{ma}$ are also shown for reference.}
    \label{fig:projs_regas}
\end{figure}

==> AAAI2023 REGAS (3)/imgs/recon_img_ablation.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{|cccccc|}
        \hline
        Phase & $\textrm{REGAS}^{\textrm{2D}}$ &  $\textrm{REGAS}^{\textrm{noRPT}}$ & $\textrm{REGAS}^{\textrm{noMA}}$ & $\textrm{REGAS}^{\textrm{noDVF}}$ & $\textrm{GT}$\\
        
        % -6$\degree$ & -3$\degree$ & 0$\degree$ (Input View) & 3$\degree$ & 6$\degree$ & 9$\degree$  \\
        1 & 
        \begin{subfigure}[b]{0.190\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_ablation/100_HM10395_07-02-2003-p4-14571_0_recon_2d.png}
            \caption{38.67/0.968}
        \end{subfigure} &
        \begin{subfigure}[b]{0.190\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_ablation/100_HM10395_07-02-2003-p4-14571_0_recon_orig.png}
            \caption{38.16/0.970}
        \end{subfigure} &
        \begin{subfigure}[b]{0.190\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_ablation/100_HM10395_07-02-2003-p4-14571_0_recon_noma.png}
            \caption{\underline{38.93/0.975}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.190\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_ablation/100_HM10395_07-02-2003-p4-14571_0_recon_ours.png}
            \caption{\bf{39.80/0.976}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.190\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_ablation/100_HM10395_07-02-2003-p4-14571_0_gt.png}
            \caption{PSNR/SSIM}
        \end{subfigure} \\
        7 & 
        \begin{subfigure}[b]{0.190\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_ablation/100_HM10395_07-02-2003-p4-14571_6_recon_2d.png}
            \caption{33.87/0.911}
        \end{subfigure} &
        \begin{subfigure}[b]{0.190\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_ablation/100_HM10395_07-02-2003-p4-14571_6_recon_orig.png}
            \caption{34.38/0.919}
        \end{subfigure} &
        \begin{subfigure}[b]{0.190\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_ablation/100_HM10395_07-02-2003-p4-14571_6_recon_noma.png}
            \caption{\underline{36.09/0.949}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.190\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_ablation/100_HM10395_07-02-2003-p4-14571_0_recon_ours.png}
            \caption{\bf{36.87/0.954}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.190\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_ablation/100_HM10395_07-02-2003-p4-14571_6_gt.png}
            \caption{PSNR/SSIM}
        \end{subfigure} \\
        \hline
    \end{tabular}
    \caption{Visual comparisons of 4D reconstructions from ablation study. The best generation metrics are bold, the second best is underlined. Metrics are calculated volume-wise.}
    \label{tab:ablation_img}
\end{figure*}

==> AAAI2023 REGAS (3)/imgs/recon_imgs.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{|c|c|ccc|ccc|cc|}
        \hline
        Phase & OSSART & U-Net & DL-PICCS & $\textrm{REGAS}^{\textrm{noDVF}}$ & $\textrm{OSSART}^{\textrm{TTV}}$  & SMEIR & REGAS & DVF-GT &GT\\
        
        1 & 
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_0_ossart.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_0_unet_sup.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_0_unet_sup_piccs.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_0_recon_ours_w_o_dvf.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_0_ossart_temporal.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_0_recon_smeir.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_0_recon_ours.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_0_recon_smeir_gt.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_0_gt.png}
        \end{subfigure} \\
         & 
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_0_ossart_diff.png}
            \caption{36.68/0.958}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_0_unet_sup_diff.png}
            \caption{36.98/0.964}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_0_unet_sup_piccs_diff.png}
            \caption{38.48/0.971}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_0_recon_ours_w_o_dvf_diff.png}
            \caption{\underline{39.80/0.976}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_0_ossart_temporal_diff.png}
            \caption{37.43/0.971}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_0_recon_smeir_diff.png}
            \caption{38.48/0.972}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_0_recon_ours_diff.png}
            \caption{\bf{42.38/0.986}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_0_recon_smeir_gt_diff.png}
            \caption{42.12/0.984}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[height=\textwidth]{imgs/diff_color/axis.png}
            \caption{PSNR/SSIM}
        \end{subfigure} \\
        \hline
        
        5 & 
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_4_ossart.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_4_unet_sup.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_4_unet_sup_piccs.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_4_recon_ours_w_o_dvf.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_4_ossart_temporal.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_4_recon_smeir.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_4_recon_ours.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_4_recon_smeir_gt.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_4_gt.png}
        \end{subfigure} \\
         & 
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_4_ossart_diff.png}
            \caption{36.12/0.952}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_4_unet_sup_diff.png}
            \caption{36.75/0.963}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_4_unet_sup_piccs_diff.png}
            \caption{38.42/0.971}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_4_recon_ours_w_o_dvf_diff.png}
            \caption{\underline{39.08/0.973}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_4_ossart_temporal_diff.png}
            \caption{37.22/0.970}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_4_recon_smeir_diff.png}
            \caption{38.70/0.974}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_4_recon_ours_diff.png}
            \caption{\bf{42.27/0.986}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_4_recon_smeir_gt_diff.png}
            \caption{42.74/0.985}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[height=\textwidth]{imgs/diff_color/axis.png}
            \caption{PSNR/SSIM}
        \end{subfigure} \\
        \hline        
        
        \hline
        8 & 
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_8_ossart.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_8_unet_sup.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_8_unet_sup_piccs.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_8_recon_ours_w_o_dvf.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_8_ossart_temporal.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_8_recon_smeir.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_8_recon_ours.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_8_recon_smeir_gt.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/imags_update/100_HM10395_07-02-2003-p4-14571_8_gt.png}
        \end{subfigure} \\
         & 
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_7_ossart_diff.png}
            \caption{32.42/0.880}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_7_unet_sup_diff.png}
            \caption{34.20/0.939}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_7_unet_sup_piccs_diff.png}
            \caption{35.13/0.941}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_7_recon_ours_w_o_dvf_diff.png}
            \caption{\underline{36.13/0.947}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_7_ossart_temporal_diff.png}
            \caption{35.56/0.953}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_7_recon_smeir_diff.png}
            \caption{35.28/0.953}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_7_recon_ours_diff.png}
            \caption{\bf{40.55/0.980}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{imgs/diff_color/100_HM10395_07-02-2003-p4-14571_7_recon_smeir_gt_diff.png}
            \caption{40.57/0.977}
        \end{subfigure} &
        \begin{subfigure}[b]{0.100\linewidth}
            \includegraphics[height=\textwidth]{imgs/diff_color/axis.png}
            \caption{PSNR/SSIM}
        \end{subfigure} \\        
        \hline
    \end{tabular}
    \caption{Visual comparisons of 4D reconstructions by different methods for phases 1 and 8. The best generation metrics are bold, the second best is underlined. Metrics are calculated volume-wise, and the difference maps are provided below the reconstruction images.}
    \label{tab:quant_img}
    \vspace{-1.5em}
\end{figure*}

==> AAAI2023 REGAS (3)/intro.tex <==
\section{Introduction}
Cone Beam Computed Tomography (CBCT) is a medical imaging technique widely adopted in dentistry, image-guided radiation therapy, etc. CBCT acquires 2D tomographic views of 3D object by emitting radiation from a rotating gantry, as shown in Fig.~\ref{CBCT_acq}, and use these views for 3D reconstruction~\cite{Feldkamp:84}. Compared to traditional CT, a CBCT scanner emits less radiation on patients~\cite{doi:10.3109/0284186X.2011.590525}, is less expensive, and is more flexible. %allowing for different postures by patients during acquisition.

% Cone Beam Computed Tomography (CBCT) is a medical imaging technique that holds several advantages over traditional CT. It acquires 2D tomographic views of the 3D object by emitting radiation from a rotating gantry, and use these views for 3D reconstruction~\cite{Feldkamp:84}. A CBCT scanner is less expensive and more flexible in design, which allows for different postures by patients during acquisition. Furthermore, a CBCT scanner emits less effective radiation on patients than a traditional CT scanner~\cite{doi:10.3109/0284186X.2011.590525} and is widely adopted in areas like dentistry and image-guided radiation therapy.
   
   
   
   
   
   %A CBCT scanner consists of an X-ray source and a planar detector mounted on a gantry. As shown in Fig. \ref{CBCT_acq}, by rotating the gantry and emitting radiation from different angles, a CBCT scanner acquires different 2D projections of the 3D object and uses those views for reconstruction \cite{Feldkamp:84}. Compared to Fan Beam CT (FBCT), a CBCT scanner is less expensive and more flexible in design, which allows for different postures by patients during acquisition. Furthermore, a CBCT scanner emits less effective radiation on patients than a traditional CT scanner \cite{doi:10.3109/0284186X.2011.590525}. As a result, CBCT is widely adopted in areas like dentistry and image-guided radiation therapy.
   
  \input{imgs/intro}
   Accurate lung CBCT imaging is of significant clinical value, especially given the Coronavirus pandemic. However, lung CBCT imaging is affected by the \textit{motion-induced} inconsistencies between acquired views and the subsequent motion artifacts in reconstructions, as shown in Fig.~\ref{FBP}. 
   A common way to address this is to model the breathing motion as a cyclical process and approximate it by a number of 3D CBCTs, referred to as \textit{phases}. Under this model, each view is attributed to one of the phases for reconstruction. The phase-view correspondence can be obtained either through dedicated physical devices~\cite{Beaudry_2015} or through signal processing on acquisition data~\cite{yan2013extracting}. This is known as respiratory-gated 4D CBCT reconstruction. While motion is disentangled by the phase dimension, each phase corresponds to only a portion of the acquired views; therefore, \textit{a high quality 4D CBCT requires a large number of views to faithfully reconstruct each phase}. This leads to a trade-off between a longer scan time and higher radiation dosage, or lower image qualities with few views, similar to a regular 3D CBCT acquisition. 
   
   
   %, which can be seen as a sparse-view CT reconstruction problem
   
   Reconstructing 4D CBCT with limited acquisitions is a difficult problem. Existing methods (\romannumeral 1) rely on handcrafted regularizers to address the aliasing artifacts, e.g. through spatial or temporal Total Variation (TV)~\cite{andersen1984simultaneous,blondiaux2017imagerie}, or (\romannumeral 2) require additional information like prior scans, air-flow volume and velocity, deformation vector field (DVF) model, etc.~\cite{brock2010reconstruction,chee2019mcsart,ren2012development,wang2013simultaneous}, which introduces additional devices and costs into the process. 
   Many deep learning based (DL-based) methods use supervised learning to suppress sparse-view artifacts, e.g. \cite{pmid32575088,DBLP:journals/tmi/HanY18,https://doi.org/10.1002/mp.15183}; however, these end-to-end methods are applicable only to 2D CT due to the heavy computational and data requirements. Furthermore, factors such as scanner differences and breathing motion differences can lead to generalization issues from supervised training. 
    

    
    
    
%   Various methods have been proposed to improve 4D CBCT reconstruction with limited acquisitions, and can be divided into two categories - the algebraic \cite{andersen1984simultaneous,blondiaux2017imagerie,qiu2012blockwise} and deformation vector field (DVF)-based approaches \cite{brock2010reconstruction,chee2019mcsart,ren2012development,wang2013simultaneous}. Algebraic methods incorporates various priors, e.g. existing scans, temporal and spatial Total Variation (TV) constraints to optimize 
   
   
   %help remove some noise in the reconstructed phases, the results are often unsatisfactory. DVF-based approaches, on the other hand, either require a high quality 4D CBCT of the same patient as a prior to estimate DVFs from, or in some cases rely on algebraic methods for initial reconstructions and thus are not guaranteed to converge in finding DVFs.
   

   
   
   %leading to irregular sparse-view reconstruction artifacts. The sparsity is also very high; for a ten-phase reconstruction, each phase on average gets a tenth of observations. As such, under an $\mathcal{L}_{1}$ objective function, existing DL-based models often lead to heavy smoothing of details. %\haofu{which methods are your talking about? add references here}
   
%   We propose a novel respiratory-gated 4D CBCT reconstruction method that leverages the advantages of both traditional and DL-based approaches. Our method, named REspiratory-GAted Synthesis of views (REGAS), aims at synthesizing the missing views in every phase. The key observations that motivate this approach are two-fold. Firstly, it is difficult to recover useful information from undersampled 3D reconstructions as details are already overlapped and thus destroyed by sparse-view artifacts. Secondly, incorporating both acquired views and the 3D reconstruction process in an end-to-end trainable CNN is clearly computationally infeasible.  Therefore, we focus on view synthesis to ameliorate sparse-view artifacts and reveal the overlapped information, leaving 3D reconstruction out of the learning pipeline. 

We propose a novel 4D CBCT reconstruction method called \underline{RE}spiratory-\underline{GA}ted \underline{S}ynthesis of views (\textbf{REGAS}), which combines the advantages of traditional methods and DL-based methods. We note that a key component to address 4D CBCT reconstruction is inter-phase deformation modeling; i.e., we can obtain high quality 4D CBCT reconstruction if the breathing DVF is known. However, obtaining such DVF is extremely difficult with limited acquisitions due to noisy reconstruction and a lack of groundtruth. To address the reconstruction, REGAS first synthesizes the unobserved views of each phase through a Convolutional Neural Network (CNN). The synthesized views are then combined with the observed views for reconstruction, which addresses the undersampled condition and the subsequent streaky artifacts. More accurate DVFs are estimated based on our improved reconstructions, and are used to further update individual phases from observed views only. %This effectively removes inconsistencies from synthesized views.

REGAS has several advantages compared to previous DL-based methods. Firstly, REGAS is \textbf{self-supervised}; it synthesizes unobserved views by leveraging the
3D geometric consistency from undersampled phases and the texture similarity to observed views, which is captured by a self-supervised adversarial loss. Furthermore, REGAS is \textbf{scalable to high resolution} through our novel Ray Path Transformation (RPT), which allows for distributed, differentiable forward projections. Therefore, REGAS can synthesize views that are \textbf{geometrically consistent and of high fidelity}, while requiring no groundtruth for training. The synthesized views lead to higher quality reconstructions, which assist in better DVF estimation. The accurate DVF estimation enables us to obtain synthesis-free reconstructions and eliminate concerns about the reliability of generative methods.












%   from 
%   by focusing on view synthesis, our method directly addresses the acquisition domain, therefore avoiding infeasible computational demands compared to if reconstruction is performed within the CNN system;
%   is not prone to the disturbance of unpredictable artifacts in the reconstructed space, thus is more robust.
%   \haofu{rephrase this sentence. the connection between view synthesis and robust to unpredictable artifacts is unclear}
%   As views from one angle are similar to those from neighboring angles, we can capture such statistical similarity through recent advances in generative adversarial networks (GANs). In accordance with imaging physics, REGAS uses a combination of 3D and 2D CNNs to follow the projection process from volumetric data. REGAS is also self-supervised, therefore does not suffer from domain shift between training and testing data. Moreover, to help address the GPU memory bottleneck that may occur while synthesizing high resolution views, we propose a novel distributed and differentiable forward projection method called Ray Path Transformation (RPT), which transforms a 3D CT into a bundle of rays along a given trajectory and organizes them into a volume. Such a volume can be easily separated and combined without affecting forward projection operations. 
   
   Our contributions can be summarized in four parts:
   
   
   %1. we can obtain a low quality version of the missing projections by re-projecting on a coarsely reconstructed phase obtained from traditional methods; 2. we can improve these projections by exploring the regional statistical similarity between the missing and observed projections, as similar approaches has become increasing reliable with the recent advances in generative adversarial networks (GANs); 3. by formulating the problem as a 2D synthesis task and leaves high dimensional reconstruction out of the DL framework, we simultaneously lower the dimension by two degrees and create the opportunity for self-supervision, as projection sample size is sufficiently large. 
   
   \begin{enumerate}
   \item We propose REGAS, which formulates respiratory-gated 4D CBCT reconstruction as a view completion problem. REGAS incorporates the physical imaging geometry with a combination of 3D and 2D CNNs.
    \item We propose a view-dependent, ray-tracing transformation scheme called RPT, which efficiently represents high resolution 3D information relating to a view and can be easily decomposed into distributed learning.
    \item We leverage the synthetic-view-assisted reconstructions for better inter-phase DVF estimations; this enable us to then optimize 4D CBCT without synthetic data and achieve more reliable performance.
    \item We evaluate REGAS on a large scale and realistically simulated CBCT acquisition data. Our experiments show that REGAS reliably reconstructs 4D CBCT from a single 3D CBCT acquisition and significantly outperforms comparable methods.
\end{enumerate}

==> AAAI2023 REGAS (3)/method.tex <==
\section{Method}

\begin{figure*}[!htb]
    \centering
      \includegraphics[width=1\textwidth]{imgs/REGAS_net.png}
    \caption{REGAS synthesizes unobserved views for phase $i$ based on observed views across all phases. It first takes the RPT transformed initial reconstructions $R^{\textrm{init}}_{i,a_k}$ and refines them through a 3D network $\mathcal{G}$. The resulting $R^{\textrm{ref}}_{i,a_k}$ forms views $P^{\textrm{ref}}_{i,a_k}$ and goes through a 2D network $\mathcal{F}$, yielding $P^{\textrm{out}}_{i,a_k}$. After training, $P^{\textrm{out}}_{i,a_k}$ are used to reconstruct $V^{\textrm{PS}}_{i}$. As a post-processing step, $V^{\textrm{PS}}_{i}$ can be used to estimate the between-phase DVFs $\mathcal{M}_{i\rightarrow j}$, which can be used to deform backprojections and allow multi-phase reconstruction based on just the observed views.}
    \label{fig:network}
    \vspace{-1.5em}
\end{figure*}
We define $P_{i,a_k}\in\mathbb{R}^{W\times H}$ as the acquired views of the $i^{\textrm{th}}$ phase $V_{i}$ along angle $a_k$, where $i\in\{1,2,...,N\}$ and $k\in\{1,2,...,K\}$. $N$ is the total number of phases that represents a complete respiratory cycle and $K$ is the total number of views acquired. Ideally, we acquire $K$ views for each phase $i$ to achieve high quality 3D reconstruction; in practice, we only acquire $K_i$ views for phase $i$, such that $K=\sum_{i}K_i$, i.e. a single 3D CBCT acquisition. Each observed view $P^{\textrm{obs}}_{\phi(a_k),a_k}$ over angle $a_k$ therefore corresponds to phase $\phi(a_k)$, where the correspondence $\phi(*)$ is measured or estimated. The goal of our proposed REGAS is to synthesize views based on $P^{\textrm{obs}}_{\phi(a_k),a_k}$ from a single CBCT acquisition, such that each phase has $K$ views for artifact reduced 4D CBCT reconstruction.


% \haofu{the previous sentences (to the beginning of this paragraph) do not seem to closely related to the context. Consider move them to section 3.2}
In the following sections, we first describe RPT, which addresses the heavy computational burden, propagates gradients between views and volumes, and enables distributed patch-based training for REGAS. We then describe the full REGAS pipeline for view synthesis. Finally, we describe how to use the REGAS reconstructions to find between-phase DVFs, which can be used for phase reconstructions where only real acquisitions $P^{\textrm{obs}}_{\phi(a_k),a_k}$ are used.


% Instead of addressing reconstruction directly in the CT domain, RGVS seeks to solve the problem by completing the projection data, i.e. such that $|a^{i}_{aug}| = K_{tot}, \forall i$ after augmentation. This is similar to the view synthesis task in nature image domain. Such a formulation allows us to use computationally intensive methods like deep learning to tackle the most direct measurements, and allow analytic 3D reconstruction, which is also computationally intensive, to happen as a post-process. 

% Many works have shown that 2D view synthesis requires a strong 3D grounding to be reliable[cite SinSyn, XraySyn]. As each phase already has several observed projections, the most intuitive approach is to do a partial 3D reconstruction and refine it through a 3D CNN, as constrained by  This presents a major challenge in computing resource, as 3D CNN has a cubic complexity and 


% We first describe our proposed Ray Path Transformation (RPT), which enables distributed patch training for a volume-projection hybrid training algorithm under a cone beam geometry. We then explain the full RGVS pipeline, which completes projection data for each phase for higher quality phase reconstruction. Finally we use these reconstructions to find between-phase DVFs, which allow us to reconstruct using only measured projections, thus allowing for maximum quality and reliability. (also explain why 3D to 2D is needed)

%This idea is similar to the dual-domain reconstruction popularly used in slice-wise CT reconstruction to reduce metal artifacts, where certain patterns are easier to be recovered from sinogram. Accurately estimating the missing projections can be formulated as a view synthesis problem, (add XraySyn in related work) where a strong knowledge of grounding in 3D is needed. As XraySyn has shown, such grounding is often computationally expensive in neural networks as dense volumetric representation. Therefore, we first describe our proposed Ray Path Transformation (RPT) module, which simultaneously serves as a differentiable forward projector and helps conserve memory.

\input{RPT}




% \subsection{Ray Path Transformation}

% RPT is proposed to address the memory bottleneck within REGAS, specifically the processing of high resolution volumetric CT in an end-to-end, 3D-to-2D CNN method. To achieve end-to-end learning, CT volumes cannot be broken down to patches as ray tracing requires full information during its traversal. The only solution without RPT is to downsample the CT volumes to compromise for GPU memory constraint, as shown in Fig. \ref{fig:RPT}. We also note that during CBCT acquisition, each view only observes a part of the volume. As such, a downsampled volume leads to significant loss in quality for each view, even though the entire volume is not needed for a particular view synthesis.


% Since every pixel on $P^{\textrm{obs}}_{i,a_k}\in\mathbb{R}^{W\times H}$ measures the projection of a ray from the light source, we consider representing the $P^{\textrm{obs}}_{i,a_k}$-observed CT volume as a series of rays. To this end, we define a ray-based representation of a CT volume $V_{\textrm{CT}}\in \mathbb{R}^{X\times Y\times Z}$ as $R\in \mathbb{R}^{W\times H\times S}$, where $S$ is the marching dimension of each ray, such that $P(w, h) = \sum_{s}R(w, h, s)$. RPT is thus defined as $\mathcal{T}(V, \psi):\mathbb{R}^{X\times Y\times Z} \to \mathbb{R}^{W\times H\times S}$ where $\psi$ includes projection parameters such as view angle $a_k$ and detector size $\{W, H\}$. As shown in Fig. , RPT records the values of rays $\bm{l}_{w,h}$ that traverse $V_{CT}$ at every marching step and organize them into a volume, which can be described as:
% \begin{align}\label{eqn: RPT}
% \begin{aligned}
%     R(w,h,s) = \mathcal{T}(V_{\textrm{CT}}, \psi) = V_{\textrm{CT}}(a^{-1}_k \bm{l}_{w,h}(s)),
% \end{aligned}
% \end{align}
% where view angle $a_k$ represents the homogeneous matrix that transforms coordinates in $V_{\textrm{CT}}$ to $\bm{l}_{w,h}$. 

% RPT has several distinct advantages: 1. it is memory-efficient in representing only the 3D context related to a particular view; 2. the transformed $R$ can be easily split and recombined over the $w-h$ plane while maintaining integrity to the forward projection process. This allows us to leverage the translational invariance of CNNs through patch learning, thus resolving the memory bottleneck in training 3D CNNs; 3. after transformation, forward projection is simplified to a summation operation along the ray marching dimension, eliminating the need for a specialized code for backpropogation; 4. by using the view-varying nature of the transformed volume, RPT serves as a form of data augmentation over the volumetric CT image. RPT is implemented through CUDA and is as fast as other GPU-implemented forward projection operations.


% To better illustrate the utility of RPT, an example is shown in Fig. 1. The acquired X-ray projections are typically of high resolution, therefore they requires a high resolution volume to capture the detail level during reconstruction. As synthesis on missing projections requires 3D context, $V^{\textrm{init}}_{i}$ is put into a CNN structure and thus memory constrained. Without RPT, we need to downsample $V^{\textrm{init}}_{i}$, which is the first degradation in quality. Furthermore, physically the detector only observes a part of the volume; as such heavy interpolations happen during forward projection, especially near the light source, hence a second degradation in quality. RPT cuts out the middle man, and directly yields the region of high resolution volume that the projection observes. Furthermore, $R$ can be separated to appropriate sizes, effectively removing memory limitation during training.


%In conception, the relationship between $R$ and $P$ is equivalent to $V$ and $P$ if parallel beam geometry is used for projection, as is done in X2CT-GAN; however, the equivalence is only true over two view angles. RPT is more generalized and can be used in real clinical reconstruction. RPT is implemented through CUDA. 

\subsection{REspiratory-GAted Synthesis (REGAS)}

To synthesize unobserved views, we would like to incorporate information from observed data. As such, we first obtain $V^{\textrm{init}}_{i}$ by performing algebraic reconstructions on $P^{\textrm{obs}}_{\phi(a_k),a_k}$, i.e. $V^{\textrm{init}}_{i} = \mathcal{H}(P^{\textrm{obs}}_{\phi(a_k),a_k})\hspace{0.3em} \forall a_k \hspace{0.3em} s.t. \hspace{0.3em} \phi(a_k)=i$, where $\mathcal{H}$ denotes methods like FBP or SART.
% \haofu{Two issues: 1) it seems that $P^{\textrm{obs}}_{\phi(a_k),a_k}$ means both a single view or a collection of all acquired views. needs separate notations for these two. 2) ``algebraic 3D reconstructions on $P^{\textrm{obs}}_{\phi(a_k),a_k}$" may be confusing (partially due to the first issue) for under-informed readers. need a clear description.}
Note that some $V^{\textrm{init}}_{i}$'s have higher quality than others, as phases have different durations and number of observed views. 

% As shown in Fig. \ref{fig:network}, REGAS is an end-to-end network that contains a 3D and a 2D CNN, which provides the context and freedom needed for synthesizing missing views. 

REGAS consists of a 3D CNN and a 2D CNN, which processes $V^{\textrm{init}}_{i}$ and the subsequent projected views over various view angles. In the first stage, the 3D CNN $\mathcal{G}$ has a 3D-UNet \cite{DBLP:conf/miccai/CicekALBR16} like architecture and uses all the reconstructed phases $V^{\textrm{init}}_{i}$ as inputs. This allows for structural information to be shared across phases, \textit{e.g.,} phase-invariant features such as the static bone structure can be shared from higher quality phases to lower quality phases. Due to the high resolution of $V^{\textrm{init}}_{i}$, training on a sufficiently deep $\mathcal{G}$ is only feasible by first transforming $V^{\textrm{init}}_{i}$ to $R^{\textrm{init}}_{i,a_k}$ through RPT and decomposing them to patches. The forward process of $\mathcal{G}$ can be described as:
\begin{align}\label{eqn: 3DCNN}
\begin{aligned}
    \{R^{\textrm{ref}}_{1,a_k},R^{\textrm{ref}}_{2,a_k},...,R^{\textrm{ref}}_{N,a_k}\}=\mathcal{G}(R^{\textrm{init}}_{\forall i,a_k}) + R^{\textrm{init}}_{\forall i,a_k}\\
    R^{\textrm{init}}_{\forall i,a_k} = R^{\textrm{init}}_{1,a_k} \oplus R^{\textrm{init}}_{2,a_k}\oplus...\oplus R^{\textrm{init}}_{N,a_k},
\end{aligned}
\end{align}
where $\oplus$ concatenates $R^{\textrm{init}}_{i,a_k}$ over the channel dimension. We can then obtain views through forward projection, i.e. $P^{\textrm{ref}}_{i,a_k} = \sum_{s}R^{\textrm{ref}}_{i,a_k}$.

The second view-refining stage consists of an RDN-based \cite{DBLP:conf/cvpr/ZhangTKZ018} 2D CNN $\mathcal{F}$, which individually processes views from each phase and can be described as: \begin{align}\label{eqn: 2DCNN}
\begin{aligned}
    P^{\textrm{out}}_{i,a_k}=\mathcal{F}(P^{\textrm{ref}}_{i,a_k})+P^{\textrm{ref}}_{i,a_k}.
\end{aligned}
\end{align} 
As described, residual learning is used in Eq. (\ref{eqn: 3DCNN}) and Eq. (\ref{eqn: 2DCNN}) to promote faster convergence.

Due to the limited data availability for supervision and the changing imaging condition, we seek to train $\mathcal{G}$ and $\mathcal{F}$ by exploring the rich information within observed views. For every $a_k$, we have one observed view, which can be used as an $\mathcal{L}_1$ reconstruction constraint with its synthesis: 
\begin{align}\label{eqn: recon_loss}
\mathcal{L}_{\textrm{rec}}=\lVert P^{\textrm{out}}_{\phi(a_k),a_k} - P^{\textrm{obs}}_{\phi(a_k),a_k}\rVert_1.
\end{align}
While we do not have observed views for other phases, we note that these phases are observed at only slightly rotated angles, if the total number of acquisitions $K$ is sufficiently dense, which is true in real applications \cite{shieh2019spare}. We therefore use a patch-wise GAN loss to constrain training on unobserved views, described as:
\begin{align}\label{eqn: 2DCNN_GAN}
\begin{aligned}
\mathcal{L}^{\mathcal{D}}_{\textrm{GAN}}(P^{\textrm{out}}_{i,a_k}, P^{\textrm{obs}}_{i,nbr(i,a_k)})&=\\
\mathbb{E}(\mathcal{D}(P^{\textrm{obs}}_{i,nbr(i,a_k)}-1)^2)) &+
\mathbb{E}(\mathcal{D}(P^{\textrm{out}}_{i,a_k}-0)^2)\\
\mathcal{L}^{\mathcal{G}}_{\textrm{GAN}}(P^{\textrm{out}}_{i,a_k})&=\mathbb{E}(\mathcal{D}(P^{\textrm{out}}_{i,a_k}-1)^2),
\end{aligned}
\end{align} 
where $nbr(i,a_k)$ yields the closest neighboring view angle from $a_k$ that observes phase $i$. %We find that a GAN formulation can leverage the strong statistical similarity between $P^{\textrm{obs}}_{i,nbr(i,a_k)}$ and $P^{\textrm{obs}}_{i,a_k}$, despite their pixel-wise difference.

Additionally, we propose a self-supervised loss at the volumetric level. We denote $V^{\textrm{ma}}$ as the motion-affected CT reconstruction by using views of all phases. $V^{\textrm{ma}}$ is blurry over regions that are moving; however, it is of high quality over static regions. As $\mathcal{G}$ generates $R^{\textrm{ref}}_{i,a}$ of all phases $i$, the voxel-wise average of these phase reconstructions similarly follows this observation; therefore, we define a motion averaging loss:
\begin{align}\label{eqn:3D_loss}
\mathcal{L}_{\textrm{MA}}=\lVert \frac{1}{N}\sum_{i}R^{\textrm{ref}}_{i,a_k} - R^{\textrm{ma}}_{a_k}\rVert_1, 
\end{align}
where $R^{\textrm{ma}}_{a_k}$ is transformed through RPT from $V^{\textrm{ma}}$ over view angle $a_k$. We find that while $\mathcal{L}_{\textrm{MA}}$ is an inexact loss due to the different reconstruction procedures, it is useful in stabilizing the network and suppressing sparse-view artifacts in $R^{\textrm{init}}_{i,a}$. The overall loss for training the full REGAS is therefore:
\begin{align}\label{eqn:overall_loss}
\mathcal{L}_{\textrm{all}}=\lambda_{\textrm{MA}}\mathcal{L}_{\textrm{MA}} + \lambda_{\textrm{rec}}\mathcal{L}_{\textrm{rec}} + \lambda_{\textrm{GAN}}\mathcal{L}_{\textrm{GAN}}, 
\end{align}
where $\lambda_{\textrm{MA}}$, $\lambda_{\textrm{rec}}$, and  $\lambda_{\textrm{GAN}}$ are weights for their respective loss, empirically chosen as 1, 0.1, and 0.05, respectively.

% Based on RPT, we describe our proposed RGVS network at synthesizing unobserved projections of a given phase. 

% As shown in Fig. 2, RGVS is an end-to-end trainable, 3D-to-2D CNN network. First, to eliminate noise and promote information sharing between initially reconstructed phases, we propose a self-supervised 3D loss called motion average loss. The idea of MAL is that the average of all phases should be similar to a reconstruction using all observed projections. 


% The high resolution volumes $V^{\textrm{init}}_{i}$ are first transformed through RPT to obtain $R^{\textrm{init}}_{i,a}$ along view angle $a$. All phases of $R^{\textrm{init}}_{i,a}$ are concatenated in the channel dimension as the input to a 3D CNN $\mathcal{G}$. Mathematically this is expressed as:
% \begin{align}\label{eqn: 3DCNN}
% \begin{aligned}
%     \{R^{\textrm{ref}}_{1,a},R^{\textrm{ref}}_{2,a},...,R^{\textrm{ref}}_{N,a}\}=\mathcal{G}(R^{\textrm{init}}_{1,a} \oplus R^{\textrm{init}}_{2,a}\oplus...\oplus R^{\textrm{init}}_{N,a}).
% \end{aligned}
% \end{align}

% This provides a signal to maintain a degree of 3D consistency and prevent collapse of the overall system - as without it the network can degrade to using the phase with the highest quality for 2D stage. Specifically the 3DCNN network can dynamically determine the proper weights voxel-wise that help establish the relationship. 
% The overall results 



\input{tables/metrics}
\subsection{Between-phase DVF Estimation}\label{sec:dvf}
After REGAS is trained to convergence, we can complete the missing views by performing inference on $V^{\textrm{init}}_{i}$ over all $a_k$. After completion, $P^{\textrm{out}}_{i,a_k}$ and $P^{\textrm{obs}}_{\phi(a_k),a_k}$ are used to reconstruct the final phases, denoted as $V^{\textrm{VS}}_{i}$. 

To further improve quality, 
%Due to the high quality of $V^{\textrm{VS}}_{i}$, 
we incorporate $V^{\textrm{VS}}_{i}$ into a \textit{DVF-based post-processing} step. To do so, we find the deformation field $\mathcal{M}_{i\rightarrow j}$ between each phase pair $<V^{\textrm{VS}}_{i},V^{\textrm{VS}}_{j}>$, using a well-performing 3D registration methods, e.g. \cite{AVANTS200826,DBLP:journals/tmi/BalakrishnanZSG19}. After obtaining DVFs, we apply a deformed FBP to reconstruct phases based on only $P^{\textrm{obs}}_{\phi(a_k),a_k}$, as shown in Fig \ref{fig:network}. Specifically, during backprojection where the filtered pixels on $P^{\textrm{obs}}_{\phi(a_k),a_k}$ are traced back to the light source, we deform ray paths according to $\mathcal{M}_{\phi(a_k)\rightarrow j}$, where $j$ is the intended phase for reconstruction. Deformed rays from all $a_k$'s are summed over the common volumetric space, yielding $V^{\textrm{DVF}}_{j}$. 

Since $V^{\textrm{DVF}}_{j}$ is reconstructed with observed data, it contains much less artifacts induced by the sparse-view condition; however, the accuracy of $V^{\textrm{DVF}}_{j}$ depends on the assumptions within the DVF reconstruction formulation, \textit{i.e.,} breathing motion is accurately modeled by DVFs. We discuss in Section \ref{sec:dvf_exp} the advantages and disadvantages of DVF-based reconstruction.

% We can then use $\mathcal{M}_{pha(a_k)\rightarrow j}$ to warp the backprojection trajectory of $P^{\textrm{obs}}_{pha(a_k),a_k}$ to all other phases $j$, thus achieve reconstructing all phases with only observed data.





==> AAAI2023 REGAS (3)/method_new.tex <==
\section{REspiratory-GAted Synthesis (REGAS)}

\begin{figure*}[!htb]
    \centering
      \includegraphics[width=1\textwidth]{imgs/REGAS_network.png}
    \caption{REGAS synthesizes unobserved views for phase $i$ based on observed views across all phases. It first takes the RPT transformed initial reconstructions $R^{\textrm{init}}_{i,a_k}$ and refines them through a 3D network $\mathcal{G}$. The resulting $R^{\textrm{ref}}_{i,a_k}$ forms views $P^{\textrm{ref}}_{i,a_k}$ and goes through a 2D network $\mathcal{F}$, yielding $P^{\textrm{syn}}_{i,a_k}$. After training, $P^{\textrm{syn}}_{i,a_k}$ are used to reconstruct $V^{\textrm{syn}}_{i}$. The RPT module generates patch separable volumes with respect to the projection angle, and is differentiable.}
    \label{fig:network}
    % \vspace{-1.5em}
\end{figure*}

Let $P^{\textrm{obs}} = \{P^{\textrm{obs}}(a_k)\}_{k=1}^K$ be $K$ views observed from a single CBCT acquisition process where $a_k$ denotes the angle of the $k^{\textrm{th}}$ view. Through respiratory gating, views of $P^{\textrm{obs}}$ can be binned into several phases with $P^{\textrm{obs}}=\cup_{i} P^{\textrm{obs}}_i$, where $P^{\textrm{obs}}_i$ denotes the set of views from phase $i$. After binning, we can reconstruct a CBCT image for phase $i$ using views from $P^{\textrm{obs}}_i$. However, since $|P^{\textrm{obs}}_i|\ll K$, the reconstructed image suffers from aliasing artifacts. At the core of REGAS, we propose to synthesize the unobserved views $P^{\textrm{syn}}_i$ for all $i$, such that $|P^{\textrm{obs}}_i|+|P^{\textrm{syn}}_i|=K$, and thus reconstructing CBCT images using $P^{\textrm{syn}}_i$ and $P^{\textrm{syn}}_i$ results in less aliasing artifact. In the following sections, we describe the two main components of REGAS: \emph{Ray Path Transformation} (RPT), which is a differentiable projection scheme that enables scalable view synthesis under the Cone-Beam geometry, and a \emph{View Synthesis Network} (VSN) that generates high quality $P^{\textrm{obs}}_i$ with self-supervision.


\input{RPT}


\subsection{View Synthesis Network (VSN)}

Two factors are essential in synthesizing reliable unobserved views for different phases. Firstly, the synthesized views of phase $i$ should be geometrically consistent with the observed views of the same phase, especially over the regions with large motion. Secondly, the synthesized views should be realistic and contain little noise in their texture. 

To ensure geometric consistency, we first obtain initial phase reconstructions $V^{\textrm{init}}_{i}=\mathcal{H}(P^{\textrm{obs}}_i)$, where $\mathcal{H}$ denotes a reconstruction method, e.g., FDK or SART. While $V^{\textrm{init}}_i$ have low imaging quality, they provide geometric templates to synthesize unobserved views. To synthesize views along angle $a_k$, we use RPT to obtain $R^{\textrm{init}}_{i,a_k}$ to reduce memory footprint. 

As shown in Fig.~\ref{fig:network}, the View Synthesis Network (VSN) consists of two subnets. The first subnet is a \underline{3D CNN $\mathcal{G}$} with a UNet-like architecture that removes artifacts in $R^{\textrm{init}}_{i,a_k}$. The forward process of $\mathcal{G}$ can be described as:
\begin{align}\label{eqn: 3DCNN}
\begin{aligned}
    \{R^{\textrm{ref}}_{1,a_k},R^{\textrm{ref}}_{2,a_k},...,R^{\textrm{ref}}_{N,a_k}\}=\mathcal{G}(R^{\textrm{init}}_{\forall i,a_k}) + R^{\textrm{init}}_{\forall i,a_k}\\
    R^{\textrm{init}}_{\forall i,a_k} = R^{\textrm{init}}_{1,a_k} \oplus R^{\textrm{init}}_{2,a_k}\oplus...\oplus R^{\textrm{init}}_{N,a_k},
\end{aligned}
\end{align}
where $\oplus$ concatenates $R^{\textrm{init}}_{i,a_k}$ over the channel dimension. The refined volumes $R^{\textrm{ref}}_{i,a_k}$ are constrained through a self-supervised loss, described as 
\begin{align}\label{eqn:3D_loss}
\mathcal{L}_{\textrm{MA}}=\lVert \frac{1}{N}\sum_{i}R^{\textrm{ref}}_{i,a_k} - R^{\textrm{ma}}_{a_k}\rVert_1, R^{\textrm{ma}}_{a_k}=\mathcal{T}(V^{\textrm{ma}}, a_k),
\end{align}
where $V^{\textrm{ma}}=\mathcal{H}(P^{\textrm{obs}})$ is the motion-affected reconstruction using all observed views. While $V^{\textrm{ma}}$ is blurry over moving anatomical regions, it is of high quality over static anatomical regions. Similarly, $R^{\textrm{ref}}_{i,a_k}$ on average should follow this pattern, espeically over empty space.

The second subnet is a \underline{2D CNN $\mathcal{F}$} based on RDN \cite{DBLP:conf/cvpr/ZhangTKZ018} that individually processes views from each phase and can be described as: \begin{align}\label{eqn: 2DCNN}
\begin{aligned}
    P^{\textrm{syn}}_{i}(a_k)=\mathcal{F}(P^{\textrm{ref}}_{i}(a_k))+P^{\textrm{ref}}_{i}(a_k),
\end{aligned}
\end{align}
where $P^{\textrm{ref}}_{i}(a_k) = \sum_{s}R^{\textrm{ref}}_{i}(a_k)$.
Residual learning is used in Eq. (\ref{eqn: 3DCNN}) and (\ref{eqn: 2DCNN}) to promote faster convergence.

Note that, for a given phase $i$, some of the synthesized views have corresponding $P^{\textrm{obs}}_{i}(a_k)$ during CBCT acquisition. We thus constraint its corresponding synthesis with an $\mathcal{L}_1$:

% While projections based on sparse-view reconstructions provide a geometrically consistent starting point, $P^{\textrm{ref}}_{i}(a_k)$ still lack quality as the reconstructions are undersampled. When a view along $a_k$ of phase $i$ is observed from acquisition, we constraint its corresponding synthesis with an $\mathcal{L}_1$ loss:
\begin{align}\label{eqn: recon_loss}
\mathcal{L}_{\textrm{rec}}=\lVert P^{\textrm{syn}}_i(a_k) - P^{\textrm{obs}}_i(a_k)\rVert_1.
\end{align}
Such a reconstruction loss also prevents Eq.~(\ref{eqn:3D_loss}) from making individual $R^{\textrm{ref}}_{i,a_k}$ the same as $R^{\textrm{ma}}_{a_k}$.

For those synthesized views without corresponding observations, an adversarial loss is employed to ensure that the synthesized views are statistically similar to the observed views of the same phase but at slightly rotated angles,
% we note that these phases are observed at only slightly rotated angles, if the total number of acquisitions $K$ is sufficiently dense, which is true in real applications \cite{shieh2019spare}. We therefore use a patch-wise GAN loss to constrain training on unobserved views, described as:
\begin{flalign}\label{eqn: 2DCNN_GAN}
\begin{aligned}
\mathcal{L}^{\mathcal{D}}_{\textrm{GAN}}=
\mathbb{E}&[\mathcal{D}(P^{\textrm{obs}}_i(a_k^*))-1)^2] +
\mathbb{E}[\mathcal{D}(P^{\textrm{syn}}_i(a_k))-0)^2],\\
\mathcal{L}^{\mathcal{G}}_{\textrm{GAN}}=\mathbb{E}&[\mathcal{D}(P^{\textrm{syn}}_i(a_k))-1)^2],
\end{aligned}
\end{flalign} 
where $P^{\textrm{obs}}_i(a_k^*)$ is a view from $P^{\textrm{obs}}_i$ and has the closet view angle $a_k^*$ to $a_k$. %We find that a GAN formulation can leverage the strong statistical similarity between $P^{\textrm{obs}}_{i,nbr(i,a_k)}$ and $P^{\textrm{obs}}_{i,a_k}$, despite their pixel-wise difference.

% Additionally, we propose a self-supervised loss at the volumetric level. We denote $V^{\textrm{ma}}$ as the motion-affected CT reconstruction by using views of all phases. $V^{\textrm{ma}}$ is blurry over regions that are moving; however, it is of high quality over static regions. As $\mathcal{G}$ generates $R^{\textrm{ref}}_{i,a}$ of all phases $i$, the voxel-wise average of these phase reconstructions similarly follows this observation; therefore, we define a motion averaging loss:
% \begin{align}\label{eqn:3D_loss}
% \mathcal{L}_{\textrm{MA}}=\lVert \frac{1}{N}\sum_{i}R^{\textrm{ref}}_{i,a_k} - R^{\textrm{ma}}_{a_k}\rVert_1, 
% \end{align}
% where $R^{\textrm{ma}}_{a_k}$ is transformed through RPT from $V^{\textrm{ma}}$ over view angle $a_k$. We find that while $\mathcal{L}_{\textrm{MA}}$ is an inexact loss due to the different reconstruction procedures, it is useful in stabilizing the network and suppressing sparse-view artifacts in $R^{\textrm{init}}_{i,a}$. 

The overall loss for training the full REGAS is therefore:
\begin{align}\label{eqn:overall_loss}
\mathcal{L}_{\textrm{all}}=\lambda_{\textrm{MA}}\mathcal{L}_{\textrm{MA}} + \lambda_{\textrm{rec}}\mathcal{L}_{\textrm{rec}} + \lambda_{\textrm{GAN}}\mathcal{L}_{\textrm{GAN}}, 
\end{align}
where $\lambda_{\textrm{MA}}$, $\lambda_{\textrm{rec}}$, and  $\lambda_{\textrm{GAN}}$ are weights for their corresponding losses, and their values are empirically chosen as 1, 0.1, and 0.05, respectively.

% Based on RPT, we describe our proposed RGVS network at synthesizing unobserved projections of a given phase. 

% As shown in Fig. 2, RGVS is an end-to-end trainable, 3D-to-2D CNN network. First, to eliminate noise and promote information sharing between initially reconstructed phases, we propose a self-supervised 3D loss called motion average loss. The idea of MAL is that the average of all phases should be similar to a reconstruction using all observed projections. 


% The high resolution volumes $V^{\textrm{init}}_{i}$ are first transformed through RPT to obtain $R^{\textrm{init}}_{i,a}$ along view angle $a$. All phases of $R^{\textrm{init}}_{i,a}$ are concatenated in the channel dimension as the input to a 3D CNN $\mathcal{G}$. Mathematically this is expressed as:
% \begin{align}\label{eqn: 3DCNN}
% \begin{aligned}
%     \{R^{\textrm{ref}}_{1,a},R^{\textrm{ref}}_{2,a},...,R^{\textrm{ref}}_{N,a}\}=\mathcal{G}(R^{\textrm{init}}_{1,a} \oplus R^{\textrm{init}}_{2,a}\oplus...\oplus R^{\textrm{init}}_{N,a}).
% \end{aligned}
% \end{align}

% This provides a signal to maintain a degree of 3D consistency and prevent collapse of the overall system - as withsyn it the network can degrade to using the phase with the highest quality for 2D stage. Specifically the 3DCNN network can dynamically determine the proper weights voxel-wise that help establish the relationship. 
% The overall results 



\input{tables/metrics_new}
\subsection{Deformation-based Refinement}\label{sec:dvf}

Combining synthesized and observed views, we can reconstruct phases $V^{syn}_i=\mathcal{H}(\{P^{\textrm{obs}}_i,P^{\textrm{syn}}_i\})$ and obtain images with less severe sparse-view artifacts. However, the detail quality of $V^{syn}_i$ is still lacking due to the imperfect synthetic views. To address this, we apply a deformation-based refinement on $V^{syn}_i$. 
%An additional deformation-based refinement step can be performed to further improve image quality. 
Specifically, we estimate the inter-phase Deformation Vector Fields (DVFs) $D_{i\rightarrow j}$ through VoxelMorph~\cite{DBLP:journals/tmi/BalakrishnanZSG19}, where $i,j$ indicate the moving and target phases. Based on $D_{i\rightarrow j}$, we perform the following optimization to refine $V^{\textrm{syn}}_i$:


\begin{align}\label{eqn:dvf_refine}
V^{\textrm{out}}_i=\argmin_{V^{\textrm{syn}}_i} \lVert P_j^{\textrm{obs}}(a_k) - A(k)D_{i\rightarrow j} V^{syn}_i\rVert_2, \forall \{k,j\},
\end{align}
where $A(k)$ is the projection matrix from angle $a_k$. This step significantly boosts the reconstruction quality as 1. synthetic views are not used in the optimization objective, and 2. the estimated $D_{i\rightarrow j}$ is of high quality due to the lack of artifacts in $V^{syn}_i$. In fact, we show by experiments that $D_{i\rightarrow j}$ is close to the upper-bound DVF estimation from groundtruth phases.  



%Such a refinement ensures that only acquired views are used, and eliminates unfaithful details produced by synthesized views. 

In summary, REGAS produces synthetic views to reduce artifacts in $V^{syn}_i$ in a self-supervised manner; It then leverages $V^{syn}_i$ to obtain reliable DVFs such that we can update the reconstructions from only acquired views. As such, REGAS allows the reconstructions to satisfy multi-view consistency from all angles without constraining them to synthetic data. 
While deformation-based refinement is not restricted to $V^{syn}$ and can be applied to $V^{init}$, we find that $V^{syn}$ is a much better initialization and leads to better results, as the optimization process in Eq.~(\ref{eqn:dvf_refine}) is non-convex. 

% as is done in SMEIR~\cite{wang2013simultaneous}, $V^{syn}$ yields higher quality DVFs and subsequently better refinement results.



% \subsection{Between-phase DVF Estimation}\label{sec:dvf}
% After REGAS is trained to convergence, we can complete the missing views by performing inference on $V^{\textrm{init}}_{i}$ over all $a_k$. After completion, $P^{\textrm{syn}}_{i,a_k}$ and $P^{\textrm{obs}}_{\phi(a_k),a_k}$ are used to reconstruct the final phases, denoted as $V^{\textrm{VS}}_{i}$. 

% To further improve quality, 
% %Due to the high quality of $V^{\textrm{VS}}_{i}$, 
% we incorporate $V^{\textrm{VS}}_{i}$ into a \textit{DVF-based post-processing} step. To do so, we find the deformation field $\mathcal{M}_{i\rightarrow j}$ between each phase pair $<V^{\textrm{VS}}_{i},V^{\textrm{VS}}_{j}>$, using a well-performing 3D registration methods, e.g. \cite{AVANTS200826,DBLP:journals/tmi/BalakrishnanZSG19}. After obtaining DVFs, we apply a deformed FBP to reconstruct phases based on only $P^{\textrm{obs}}_{\phi(a_k),a_k}$, as shown in Fig \ref{fig:network}. Specifically, during backprojection where the filtered pixels on $P^{\textrm{obs}}_{\phi(a_k),a_k}$ are traced back to the light source, we deform ray paths according to $\mathcal{M}_{\phi(a_k)\rightarrow j}$, where $j$ is the intended phase for reconstruction. Deformed rays from all $a_k$'s are summed over the common volumetric space, yielding $V^{\textrm{DVF}}_{j}$. 

% Since $V^{\textrm{DVF}}_{j}$ is reconstructed with observed data, it contains much less artifacts induced by the sparse-view condition; however, the accuracy of $V^{\textrm{DVF}}_{j}$ depends on the assumptions within the DVF reconstruction formulation, \textit{i.e.,} breathing motion is accurately modeled by DVFs. We discuss in Section \ref{sec:dvf_exp} the advantages and disadvantages of DVF-based reconstruction.

% We can then use $\mathcal{M}_{pha(a_k)\rightarrow j}$ to warp the backprojection trajectory of $P^{\textrm{obs}}_{pha(a_k),a_k}$ to all other phases $j$, thus achieve reconstructing all phases with only observed data.





==> AAAI2023 REGAS (3)/related_work.tex <==
\section{Related Work}

% \begin{figure*}[!htb]
%     \centering
%       \includegraphics[width=1\textwidth]{imgs/RGVS_RPT.png}
%     \caption{Without RPT, a high resolution CT $V^{\textrm{HR}}$ needs to be downsampled to $V^{\textrm{LR}}$ to fit into a deep 3D CNN. Our proposed Ray Path Transformation (RPT) efficiently transform $V^{\textrm{HR}}$ to $R^{\textrm{HR}}_{a}$ based on the cone beam projection geometry. $R^{\textrm{HR}}_{a}$ is a collection of rays and thus can be separated into patches, processed by 3D CNNs, and summed over $s$ ray marching steps, while preserving the ray tracing integrity. As such, RPT enables distributed training at scale under a memory constraint.}
%     \label{fig:RPT}
%     \vspace{-1em}
% \end{figure*}
\subsection{Traditional 4D CBCT Reconstruction}

In its fundamental form, 4D CBCT reconstruction is based on the FDK algorithm~\cite{Feldkamp:84}. Under the respiratory-gated model, various methods have been proposed to improve 4D CBCT reconstruction. The algebraic approach attempts to improve reconstructions iteratively based on different aspects of image quality and can be generally described as:
\begin{align}\label{eqn:iter_recon}
\hat{V} = \argmin_V ||AV - P||^2 + R(V),
\end{align}
where $V$ is the reconstructed phase, $A$ is the the projection matrix that describes the voxel-pixel correspondence between $V$ and views $P$, and $R(V)$ is a regularization term, \textit{e.g.,} total variation (TV). The family of Algebraic Reconstruction Rechniques (ART) \cite{blondiaux2017imagerie}, such as SART and OSSART, falls under this category. Prior Image Constraint Compressive Sensing (PICCS) \cite{chen2008method} seeks to minimize the total variation and pixel-wise difference between reconstructed phase and a prior image, which can be a prior scan or the reconstruction from using all the observed views.~\cite{Ritschl_2012} propose to enforce total variation along the temporal axis. ~\cite{mory2014cardiac} propose ROOSTER, which uses various regularizations to reduce noise within a selected region of interest.

DVF-based approaches seek to use the deformation fields between phases to improve reconstructions; however, additional information is often required to find such DVFs. \cite{brock2010reconstruction,ren2012development} rely on a previously obtained high-quality 4D CT scan to compute the initial DVFs, and correct them with the currently observed views; the final DVFs are then used to deform the prior high-quality 4D scan to represent patient's current state. Combinations of algebraic and DVF-based approaches also exist, with algorithms such as SMEIR~\cite{wang2013simultaneous} and MC-SART~\cite{chee2019mcsart}. These methods obtain the initial phase reconstructions from an algebraic approach, estimate DVF based on those reconstructions, and iteratively improve both the reconstructions and the DVFs. As initial reconstructions are of low quality, there is no guarantee that DVFs and reconstructions converge simultaneously. In particular, MC-SART requires additional devices to measure diaphragm amplitude and velocity.

\subsection{Deep Learning-based CT Reconstruction}
Deep learning-based methods have obtained impressive results on reconstructing sparse-view CT images~\cite{pmid32575088,DBLP:journals/tmi/HanY18,https://doi.org/10.1002/mp.15183}. However, these methods are often designed for 2D slice reconstruction, where the computational complexity is reasonable. These methods also rely on supervised training and high quality groundtruth, which limit their application in 4D CBCT as the breathing motion is continuous and does not have an easily measurable groundtruth. 4D-AirNet~\cite{pmid32575088}, for example, performs their experiments on 2D CT slices despite motivated by 4D CBCT, as the computational cost is otherwise infeasible. 


% \subsection{GAN?}

==> AAAI2023 REGAS (3)/tables/ablation.tex <==
% \captionsetup[subfigure]{labelformat=empty}
% \vspace{-1em}
\begin{table}[!htb]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{8pt}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
     Method & $\mathcal{G}$&RPT&$\mathcal{L}_{\textrm{MA}}$& Avg. Perf. \\
    \hline
    
   
    $\textrm{REGAS}^{\textrm{2D}}$ 
    & \ding{55}
    & \ding{55}
    & \ding{55}
    & 36.09/0.938%34.7/.926
    \\
    \hline
    $\textrm{REGAS}^{\textrm{noRPT}}$
    & \ding{51}
    & \ding{55}
    & \ding{51}
    & 36.49/0.946
    \\
    \hline
    $\textrm{REGAS}^{\textrm{noMA}}$ 
    & \ding{51}
    & \ding{51}
    & \ding{55}
    & 37.96/0.964%.952
    \\
    \hline
    $\textrm{REGAS}^{\textrm{noDVF}}$ 
    & \ding{51}
    & \ding{51}
    & \ding{51}
    & 39.05/0.970\\
    \hline
    
% 2d
% &  39.10176177226589
% &  38.16367424508926
% &  34.664451454200254
% &  38.09443854597445
% &  38.34348632270469
% &  35.44613682188642
% &  34.283193137637355
% &  32.67019512928101
% &  35.1058167566285
% &  34.98395549439211

% % noMA
%   39.59167002560011+
%   39.33611142192835+
%   37.13318860401703+
%   39.11687660244069+
%   39.36898214013385+
%   37.67062106119244+
%   36.90563448432519+
%   35.60268519720126+
%   37.48310237870412+
%   37.39549065756544
% ours
%   40.60247946778495+
%   40.20440016536319+
%   38.83228371889445+
%   39.97044159884694+
%   40.11754128115322+
%   39.13486660438144+
%   37.88948706509583+
%   36.79508839307156+
%   38.51924592636906+
%   38.464886377896285

% orig
%   38.84526531732484+
%   38.075830576479056+
%   35.368587666384684+
%   37.86079509937788+
%   38.27451727017986+
%   36.06794381789527+
%   35.042745595924075+
%   34.07831657747968+
%   35.89349315217933+
%   35.3688150367625

%   0.9735371876442936+
%   0.9634434045006989+
%   0.9372570880406641+
%   0.961773893310628+
%   0.9657535808564511+
%   0.9421203655045308+
%   0.926687693117246+
%   0.9121824861323587+
%   0.9393954194800561+
%   0.9326618813735045

    
%   0.9706698385338807+
%   0.9644112657853554+
%   0.9226253089989762+
%   0.9635169526317695+
%   0.9659679177032798+
%   0.9353853750649257+
%   0.915231864588987+
%   0.885373507989508+
%   0.9275399824839033+
%   0.9270074696565473
% noMA
%   0.9778371542785732+
%   0.9747717722599083+
%   0.9584253557436109+
%   0.9745357678711001+
%   0.9759690394484254+
%   0.9636159409192316+
%   0.9555161136757274+
%   0.9377206740388481+
%   0.9604041080339477+
%   0.9601699877982676
    
    \end{tabular}\\
    \caption{Ablation comparison among different implementations of REGAS. The average performance across all phases is presented.}
    \label{tab:ablation}
    \vspace{-1.3em}
\end{table}

==> AAAI2023 REGAS (3)/tables/metrics.tex <==
\begin{table*}[!htb]
\setlength{\tabcolsep}{1pt}
\centering 
\begin{tabular}{| l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
 Phase & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9& 10 &Average\\
\hline
OSSART 
& 35.1/.942
& 34.4/.933
& 31.7/.870
& 34.3/.927 
& 34.5/.934
& 32.1/.883 
& 31.4/.864 
& 30.4/.835 
& 32.0/.879 
& 31.8/.872
& 32.8/.894\\

% $\textrm{UNet}^{small}_{sup}$ 
% & 34.9/.945
% & 34.7/.945
% & 34.0/.835
% & 34.8/.945
% & 34.8/.946
% & 34.4/.940
% & 33.8/.933
% & 33.4/.928
% & 34.2/.936
% & 34.2/.938
% \\

$\textrm{UNet}_{\textrm{sup}}$ 
& 36.7/.959
& 36.6/.959
& 35.2/.946
& 36.6/.958
& 36.7/.960
& 35.7/.952
& 34.8/.942
& 34.1/.935
& 35.4/.944
& 35.5/.949
& 35.7/.950
\\

$\textrm{REGAS}_{\textrm{2D}}$ 
&  37.6/.966
&  36.7/.958
&  33.4/.909
&  36.7/.957
&  36.9/.960
&  34.2/.922
&  33.0/.899  
&  31.2/.864
&  33.7/.913
&  33.8/.914
&  34.7/.926
\\
$\textrm{REGAS}_{\textrm{noRPT}}$
&  37.1/.965
&  36.5/.959
&  34.1/.923
&  36.4/.956
&  36.7/.960
&  34.8/.936  
&  33.8/.915
&  32.5/.894
&  34.5/.929
&  34.2/.926
&  35.1/.936
\\
$\textrm{REGAS}_{\textrm{noMA}}$ 
&  37.5/.967
&  37.2/.965
&  35.7/.946
&  37.1/.964
&  37.3/.964            
&  36.1/.952
&  35.5/.944
&  34.3/.923
&  35.8/.950
&  35.8/.948
&  36.2/.952
\\
$\textrm{REGAS}$ 
&  \bf{39.1/.977}
&  \bf{38.7/.974}
&  \bf{37.6/.964}
&  \bf{38.5/.973}
&  \bf{38.7/.974}
&  \bf{37.8/.966}      
&  \bf{36.9/.957}
&  \bf{35.5/.938}
&  \bf{37.4/.964}
&  \bf{37.4/.964}
&  \bf{37.8/.965}
\\
\hline
\hline
% FBP & N/A & &&&&&&&&\\
$\textrm{OSSART}^{\textrm{DVF}}$ & 39.0/.974 
& 39.0/.973
& 37.4/.969
& 39.1/.973
& 39.1/.971
& 37.5/.968
& 35.9/.960
& 34.3/.943
& 37.3/.965
& 37.4/.967
& 37.6/.966
\\
$\textrm{UNet}^{\textrm{DVF}}_{\textrm{sup}}$ 
& 40.2/.980
& 40.8/.980
& 40.1/.982
& 40.3/.978
& 39.5/.975
& 38.3/.977
& 37.6/.975
& 37.3/.971
& 39.9/.978
& 39.7/.979
& 39.4/.978
\\
$\textrm{REGAS}^{\textrm{DVF}}$ 
& \bf{41.8/.984} 
& \bf{42.3/.984}
&\bf{42.6/.988}
&\bf{41.8/.982}
&\bf{41.6/.980}
&\bf{41.3/.985}
&\bf{40.9/.984}
&\bf{40.1/.981}
&\bf{41.3/.982}
&\bf{41.8/.985}
&\bf{41.6/.983}
\\
\hline
\end{tabular}
\caption{Quantitative evaluation of 4D RG-CBCT reconstruction on 4D Lung~\protect\cite{2017A} in terms of PSNR and SSIM. The best results are in {\bf bold} in both algebraic and DVF-based reconstructions. Phases that have more observed views have higher PSNRs in their OSSART reconstructions.}
\vspace{-1em}
% , and the second best results are \underline{underlined}.}
\label{tab:sota_table}
\end{table*}

==> AAAI2023 REGAS (3)/tables/metrics_new.tex <==
\begin{table*}[!htb]
\setlength{\tabcolsep}{1pt}
\centering
\begin{tabular}{| l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
 Phase & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9& 10 &Average\\
\hline


OSSART 
& 37.4/.962
& 36.8/.956
& 34.3/.917
& 36.6/.953
& 36.8/.956
& 34.8/.923
& 34.0/.910
& 33.0/.889
& 34.8/.924
& 34.5/.918
& 35.3/.931
\\



U-Net
&  37.4/.966
&  37.4/.967 
&  35.7/.953
&  37.3/.967
&  37.4/.967
&  36.3/.959
&  35.4/.951
&  34.7/.943
&  36.0/.955
&  36.0/.956
&  36.4/.959
\\

DL-PICCS
&  39.0/.972
&  38.9/.973
&  36.9/.959
&  38.8/.972
&  39.0/.973
&  37.5/.965
&  36.5/.953
&  35.5/.945
&  37.0/.956
&  37.3/.962
&  37.6/.963
\\



$\textrm{REGAS}^{\textrm{noDVF}}$
&40.6/.980
&40.2/.978
&38.8/.970
&40.0/.977
&40.1/.977
&39.1/.974
&37.9/.961
&36.8/.951
&38.5/.966
&38.5/.966
&39.1/.970
\\

\hline
\hline


$\textrm{OSSART}^{\textrm{TTV}}$ 
&  38.3/.975
&  38.2/.975
&  37.6/.971
&  38.0/.974
&  38.1/.974
&  37.2/.968
&  36.7/.962
&  36.4/.958
&  36.5/.959
&  36.2/.954
&  37.3/.967
\\

SMEIR
&39.9/.977
&39.6/.977
&38.5/.973
&40.0/.978
&39.7/.977
&38.6/.973
&37.5/.968
&36.0/.958
&38.3/.971
&38.2/.971
&38.6/.972
\\



REGAS

&\bf{43.6/.989}
&\bf{43.4/.988}
&\bf{42.8/.987}
&\bf{43.6/.989}
&\bf{43.4/.988}
&\bf{42.4/.986}
&\bf{41.8/.984}
&\bf{41.2/.982}
&\bf{42.4/.986}
&\bf{42.1/.985}
&\bf{42.7/.986}
\\

\hline
DVF-GT

&43.8/.987
&43.9/.987
&43.3/.986
&44.1/.988
&43.8/.987
&42.9/.985
&42.5/.984
&41.9/.982
&43.1/.985
&43.0/.985
&43.3/.986
\\
\hline

\end{tabular}
\caption{Quantitative evaluation of 4D CBCT reconstruction on 4D Lung~\protect\cite{2017A} in terms of PSNR and SSIM. The best results are in {\bf bold} besides the reference DVF-GT. Phases that have more observed views have higher PSNRs in their OSSART reconstructions.}
% \vspace{-1.5em}
% , and the second best results are \underline{underlined}.}
\label{tab:sota_table}
\end{table*}

==> AAAI2023 REGAS (3)/tables/temp.tex <==
\begin{table*}[!htb]
\setlength{\tabcolsep}{1pt}
\centering 
\begin{tabular}{|c|ccc|ccc|ccc|ccc|}
\hline
 Method & \multicolumn{3}{c|}{DiNTS} & \multicolumn{3}{c|}{Meta-Oneshot} & \multicolumn{3}{c|}{DiNTS} & \multicolumn{3}{c|}{Meta-Oneshot} \\
\hline
Memory
& \multicolumn{3}{c|}{5067MiB}
& \multicolumn{3}{c|}{5358MiB}
& \multicolumn{3}{c|}{8802MiB}
& \multicolumn{3}{c|}{7168MiB} \\
\hline

& DSC1
& DSC2
& Avg.
& DSC1
& DSC2
& Avg.
& DSC1
& DSC2
& Avg.
& DSC1
& DSC2
& Avg.
\\
\hline
Pancreas 
& 77.41
& 47.51
& 62.46
& \bf{78.90}
& \bf{50.22}
& \bf{64.56}
& 80.06
& 52.53
& 66.29
& \bf{80.10}
& \bf{53.47}
& \bf{66.79}
\\
\hline
Liver
& 93.42
& 50.26
& 71.84
& \bf{93.95}
& \bf{56.97}
& \bf{75.46}
& \bf{94.32}
& 57.64
& 75.98
& 94.21
& \bf{57.77}
& \bf{75.99}
\\
\hline
\end{tabular}
\caption{Compared to DiNTS, our proposed Meta-Oneshot finds better structures. Specifically, our small compute model performs much better than DiNTS', and our large compute model is competitive with DiNTS' with less memory usage.}
\vspace{-1em}
% , and the second best results are \underline{underlined}.}
\label{tab:sota_table}
\end{table*}

==> AAAI2023 REGAS (3)/tables/temp_multi.tex <==
\begin{table*}[!htb]
\setlength{\tabcolsep}{1pt}
\centering 
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
 Method & \multicolumn{3}{c|}{DiNTS} & \multicolumn{3}{c|}{Meta-Oneshot} & \multicolumn{3}{c|}{MT-Meta-Oneshot} \\
\hline
Memory
& \multicolumn{3}{c|}{8802MiB}
& \multicolumn{3}{c|}{7168MiB}
& \multicolumn{3}{c|}{7000MiB} \\
\hline

& DSC1
& DSC2
& Avg.
& DSC1
& DSC2
& Avg.
& DSC1
& DSC2
& Avg.
\\
\hline
Pancreas 
& 80.06
& 52.53
& 66.29
& \bf{80.10}
& 53.47
& \bf{66.79}
& 79.85
& \bf{53.65}
& 66.75
\\
\hline
Liver
& 94.32
& 57.64
& 75.98
& 94.21
& 57.77
& 75.99
& \bf{94.39}
& \bf{58.84}
& \bf{76.62}
\\
\hline
Hepatic Vessel
& 60.85
& 66.96
& 63.91
& 60.80
& 66.72
& 63.76
& \bf{61.59}
& \bf{69.93}
& \bf{65.76}
\\
\hline
\end{tabular}
\caption{Our Multi-Task (MT) Meta-Oneshot model provides additional improvements by using a single model for a combined dataset of three different tasks. Particularly, by sharing weights for three tasks, we reduce training time by $50\%$ compared to individual training; furthermore, we observe performance improvements on the Liver and Hepatic Vessel datasets, and competitive performance over the Pancreas dataset.}
\vspace{-1em}
% , and the second best results are \underline{underlined}.}
\label{tab:sota_table}
\end{table*}

==> experiments.tex <==
\section{Experiments}
\textbf{Dataset.} Evaluating the effectiveness of respiratory-gated CBCT reconstruction on real acquisition data has some major challenges: 1. there is no gold-standard groundtruth for unobserved views of a phase due to constant breathing motion; 2. CBCT images are acquired with low dosage and tend to be noisy; 3. due to the enormous file sizes of 4D acquisition data, public dataset for respiratory-gated CBCT is scarce and only from very few patients, e.g. five cases in SPARE \cite{shieh2019spare} on the Varian system. As a proof-of-concept, we use the 4D Lung dataset from Hugo et. al.\cite{2017A}, which contains 62 high quality ten-phased 4D FBCTs, to perform experiments based on realistic simulations. Specifically, we synthesize $P_{i,a_k}$ as Digitally Reconstructed Radiographs (DRRs) \cite{milickovic2000ct} by using the projection geometry from real respiratory-gated acquisitions in SPARE. We set detector size to $\{W=256,H=192\}$, detector spacing to $1.55mm$, and the total number of acquired views to $K=680$. CT volumes are normalized to an isotropic resolution of $1.5mm$ and a resolution of $128\times256\times256$. The phase-view correspondences $\phi(*)$ are from real measurements in SPARE after aligning the max-inhale and max-exhale phases with \cite{2017A}. We use OSSART to obtain $V^{\textrm{init}}_{i}$. For RPT, the ray marching dimension is set to $S=128$; during training $R^{\textrm{init}}_{i,a_k}$ are separated into patches of $128\times128\times128$. 

%This FBCT-simulated setup also allows us to study the effectiveness of CNN-based transfer learning for RG-CBCT reconstruction without a significant domain gap. We use the LIDC-IDRI dataset[], which contains 890 lung FBCT volumes after pre-processing, to simulate the low quality reconstructions due to irregular sparse-view sampling in RG-CBCT.

% \subsection{Implementation Details}
% REGAS is trained end-to-end. For 3D CNN, REGAS uses a 3D-UNet \cite{DBLP:conf/miccai/RonnebergerFB15} structure, where five downsampling and upsampling CNN layers are used. A 2D Residual DenseNet (RDN \cite{DBLP:conf/cvpr/ZhangTKZ018}) is used for the projection-refining stage, where we use ten residual dense blocks, each of which has six convolution layers and growing rate of thirty-two. We use the ANTs package for DVF estimation, specifically by using cross correlation as the regression loss. We use TIGRE for OSSART reconstruction. We train all the models with Adam
% optimization, with a momentum of 0.5 and a learning rate of 0.0001, until they converge. For more about model architectures, please refer to the Supplemental Material. 

\input{imgs/recon_imgs}
\textbf{Baselines.} We examine the effectiveness of RPT and each component within the network structure by experimenting alternative implementations, including:

\begin{itemize}
\item $\textrm{REGAS}_{\textrm{2D}}$: We remove $\mathcal{G}$ of REGAS, and use only $\mathcal{F}$ to improve the quality of unseen views directly from $V^{\textrm{init}}_{i}$; we use losses described in Eq. (\ref{eqn: recon_loss}) and (\ref{eqn: 2DCNN_GAN}).
\item $\textrm{REGAS}_{\textrm{noMA}}$: We use REGAS without the motion averaging loss in Eq. (\ref{eqn:3D_loss}).
\item $\textrm{REGAS}_{\textrm{noRPT}}$: We use REGAS without RPT, i.e. providing $V^{\textrm{init}}_{i}$ as inputs to $\mathcal{G}$ and perform forward projection on the output volume; we then use $\mathcal{F}$ to improve synthesized view quality. $V^{\textrm{init}}_{i}$ is bicubically downsampled to $128\times128\times128$ due to memory constraint. 
% \item $\textrm{REGAS}_{DVF}$: We use REGAS with the DVF-based post-processing described in section \ref{sec:dvf}.
\end{itemize}


 We also study the effectiveness of the mainstream DL-based sparse-view reconstruction approaches, which use CNNs to recover artifact-free images from the sparse-view affected reconstructions through supervised learning. As we use 4D FBCTs for simulation and testing, we can use a CNN to train on an external FBCT dataset without suffering from a large domain gap during testing. Note that this is a \emph{theoretical} exercise; in reality it is extremely difficult to obtain artifact free, high quality CBCT groundtruth in large scale. LIDC-IDRI \cite{armato2011lung}, which contains 890 FBCT lung images after pre-processing, is used to simulate sparse-view reconstructions for training data. For fair comparison, we use 3D-UNet \cite{DBLP:conf/miccai/CicekALBR16} as the network architecture, and an $\mathcal{L}_{1}$ reconstruction loss for training. We denote such a baseline as $\textrm{UNet}_{\textrm{sup}}$. Quantitatively, we use Peak Signal-to-Noise Ratio (PSNR) and Structural SIMilarity (SSIM) \cite{DBLP:journals/tip/WangBSS04} to measure performance. Additional discussions about data processing, simulation, and other implementation details are available in the supplemental material section.
 
 
 
%  $\textrm{UNet}_{\textrm{sup}}$ follows the general approaches of [][][], which recover artifact-free images from the sparse-view affected inputs by using a CNN learned through supervision. As our experiments are performed on simulated data on FBCTs, it allows us to study the effectiveness of $\textrm{UNet}_{\textrm{sup}}$ for RG-CBCT reconstruction without a significant domain gap. For fair comparison, we use $\mathcal{G}$ in REGAS as the network for $\textrm{UNet}_{\textrm{sup}}$, and train it on the simulated data based on the LIDC-IDRI dataset. The simulation is performed according to that of 4D FBCTs used for inference and described in section \ref{sec:data}. 
% note that $K_{7}=40$, thus phase 7 is severely undersampled
% \input{imgs/projs}

% \input{imgs/dvf_imgs}
\subsection{Quantitative Evaluation}
We summarize the performance of different reconstruction approaches in Table \ref{tab:sota_table} and visualize the results in Fig. \ref{tab:ablation_img} over different phases. As we can see, due to limited and irregular sparse-view sampling, artifacts are quite severe in OSSART. In particular, we observe that some bone structural details are completely lost in phase 7. 
Due to severe sparse-view artifacts, $\textrm{UNet}_{\textrm{sup}}$ cannot recover these details in the reconstructed image domain. In fact, $\textrm{UNet}_{\textrm{sup}}$ generally oversmoothes the inputs due to training with $\mathcal{L}_{1}$ loss; consequently, even bone details that are observable through OSSART are lost in reconstructions by $\textrm{UNet}_{\textrm{sup}}$. We also observe that $\textrm{UNet}_{\textrm{sup}}$ can mistake sparse-view artifacts for real tissues and produce unfaithful details. As such, $\textrm{UNet}_{\textrm{sup}}$ is clinically unreliable despite its relatively high performance in PSNR. $\textrm{REGAS}_{\textrm{2D}}$ directly applies the 2D part of REGAS on views from $V^{\textrm{init}}_{i}$; however, these views can be very blurry due to undersampled reconstruction. Therefore, it is difficult for networks to recover views that are consistent with the underlying geometry. While $\textrm{REGAS}_{\textrm{noRPT}}$ performs slightly better than $\textrm{REGAS}_{\textrm{2D}}$ both quantitatively and visually, its information loss due to downsampling in 3D leads to lost details in 2D views and requires $\mathcal{F}$ to recover them via GAN. $\textrm{REGAS}_{\textrm{noMA}}$ shows good performance compared to the other two ablated methods, but does not share patterns as well as the full REGAS in 3D due to the lack of $\mathcal{L}_{\textrm{MA}}$. We show an instance of the synthesized views in Fig \ref{fig:proj} for all versions of REGAS. In particular, we can see that views from $\textrm{REGAS}_{\textrm{noRPT}}$ and $\textrm{REGAS}_{\textrm{noMA}}$ both recover the rib cage frame on the right side of the lung. Compared to the full REGAS, there is less clarity over the heart region in $\textrm{REGAS}_{\textrm{noMA}}$ due to the noisier 3D CTs, and $\textrm{REGAS}_{\textrm{noRPT}}$ generates more fictitious details. The full REGAS produces a much more stable and geometrically consistent synthesis, thus demonstrating the utility of each component and the effectiveness of scaling computation complexity with distributed forward projections. Please refer to the supplemental material on how volumetric resolution impacts views visually and other intermediate results.

Ideally, the synthesized views should be reintroduced to the 4D reconstruction space and updated, which helps reduce geometric inconsistencies; however, such a step is infeasible due to computing limitations. Since the 4D reconstruction space is too large to be addressed at a voxel level, DVF-based reconstruction provides an alternative solution that is less sensitive to per-voxel accuracy. 
\subsection{Deformed FBP Reconstruction}\label{sec:dvf_exp}
We apply the DVF-based post-processing described in section \ref{sec:dvf} on REGAS-reconstructed $V^{\textrm{VS}}_{i}$ to obtain $V^{\textrm{DVF}}_{i}$ through SyN \cite{AVANTS200826}. Similar post-processing can be applied to OSSART and ${\textrm{UNet}}_{\textrm{sup}}$, where we replace $V^{\textrm{VS}}_{i}$ with their respective reconstructions to find between-phase DVFs. These methods are denoted as $\textrm{REGAS}^{\textrm{DVF}}$, $\textrm{OSSART}^{\textrm{DVF}}$, and $\textrm{UNet}^{\textrm{DVF}}_{\textrm{sup}}$. Quantitative measurements are shown in Table \ref{tab:sota_table}, and visualizations are shown in Fig. \ref{tab:dvf_img}.  
Clearly, using real views for reconstruction eliminates a significant amount of streaking artifacts from the inaccuracies in synthesized views. However, artifacts induced by erroneous DVFs exist. By using bones as static markers, we can observe that results from $\textrm{OSSART}^{\textrm{DVF}}$ deform randomly from phase to phase due to unreliable DVFs, as indicated by the orange arrows. Such deformations are also observable in $\textrm{UNet}^{\textrm{DVF}}_{\textrm{sup}}$ to a lesser extent, as shown in the blurry spine reconstruction. In particular, as $\textrm{UNet}_{\textrm{sup}}$ tends to blur out details, the estimated DVFs can globally drift in the direction of the motion, as indicated by the yellow arrow in Fig. \ref{tab:dvf_img}.
In comparison, $\textrm{REGAS}^{\textrm{DVF}}$ estimates more accurate DVFs and produces higher definition reconstructions, where deformations only happen to motion-affected area.




% despite high PSNR measurements. As results from REGAS are of much higher quality, $\textrm{REGAS}^{\textrm{DVF}}$ is more stable. 

% use bones as static markers and find they shift significantly from phase to phase in results from $\textrm{OSSART}^{\textrm{DVF}}$ and, to a smaller degree, from $\textrm{UNet}^{\textrm{DVF}}_{\textrm{sup}}$, as indicated by the orange arrows in Fig. \ref{tab:dvf_img}. 
We note that minor drifts of otherwise static structures, e.g. the bones, are hard to be completely avoided for DVF-based reconstruction, as the estimated DVFs will be imperfect in describing the breathing motion even from groundtruth phases. In comparison, reconstructions from the vanilla REGAS do not suffer from this problem as convolutions do not produce geometric changes on synthesized views. Despite lower PSNR metrics, the vanilla REGAS may be preferable over $\textrm{REGAS}^{\textrm{DVF}}$ in certain scenarios. Please refer to the supplemental material for animated results of $\textrm{OSSART}^{\textrm{DVF}}$ and $\textrm{REGAS}^{\textrm{DVF}}$.

REGAS can be incorporated into iterative DVF-based methods, such as SMEIR \cite{wang2013simultaneous} and MC-SART \cite{chee2019mcsart}, in place of SART as the initial DVF-based reconstruction. As REGAS significantly reduces noise in reconstructed CBCTs, iterative DVF-based methods can benefit from fewer iterations and higher likelihood of convergence. Furthermore, it is likely that an iterative version of REGAS, where $V^{\textrm{init}}_{i}$ are replaced with reconstructed $V^{\textrm{VS}}_{i}$ from a previous iteration, can further enhance performance. REGAS also has a potential advantage in its application on real CBCT acquisition; specifically, traditional methods that derive from ART-based reconstructions use DRR to generate views, thus they suffer from a significant domain gap as DRR does not simulate real projections well \cite{DBLP:journals/corr/abs-2012-02407,DBLP:conf/miccai/UnberathZLBFAN18}. In comparison, REGAS has a view-refining CNN $\mathcal{F}$ that is GAN-based, and should help reduce such domain gaps. We plan to apply REGAS on real CBCT acquisitions in a future study.




%Note that this is different from methods such as SMEIR in a few ways: 1. there is no iteration as we can immediately obtain high quality DVFs; however, it is feasible that incorporation of iterative methods like SMEIR can help us find better DVFs; 2. reconstruction is done by warping each projection to every phase. In methods like SMEIR, due to computational complexity and issues in convergence, only $\mathcal{M}_{0\rightarrow j}$ are calculated. As the estimated DVFs likely cannot perfectly describe the transitions between phases, we find a larger number of DVF estimations leads to more accurate reconstructions.


% $\textrm{REGAS}_{\textrm{noRPT}}$, and REGAS, denoted as $\textrm{OSSART}^{\textrm{DVF}}$, $\textrm{REGAS}^{\textrm{DVF}}_{\textrm{noRPT}}$, and $\textrm{REGAS}^{\textrm{DVF}}$.

==> imgs/dvf_imgs.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{|ccccc|}
        \hline
        Phase & $\textrm{OSSART}^{\textrm{DVF}}$& $\textrm{UNet}^{\textrm{DVF}}_{\textrm{sup}}$&$\textrm{REGAS}^{\textrm{DVF}}$ & $\textrm{GT}$\\
        %&$\textrm{OSSART}^{DVF}_{sag}$&$\textrm{RG-Syn}^{DVF}_{sag}$ & $\textrm{GT}_{sag}$\\
        
        % -6$\degree$ & -3$\degree$ & 0$\degree$ (Input View) & 3$\degree$ & 6$\degree$ & 9$\degree$  \\
        2 & 
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ossart_cor_1_arrow.png}
            \caption{\hspace{4em}38.62/0.970}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ossart_sag_1.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/sup_cor_1.png}
            \caption{\hspace{4em}40.27/0.977}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/sup_sag_1.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ours_cor_1.png}
            \caption{\hspace{4em}\bf{41.79/0.982}}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ours_sag_1.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&        
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/gt_cor_1.png}
            \caption{\hspace{4em}PSNR/SSIM}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/gt_sag_1.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}\\
        
        7 & 
        
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ossart_cor_6_arrow.png}
            \caption{\hspace{4em}35.09/0.983}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ossart_sag_6.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/sup_cor_6_arrow.png}
            \caption{\hspace{4em}36.33/0.970}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/sup_sag_6_arrow.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ours_cor_6.png}
            \caption{\hspace{4em}\bf{40.89/0.982}}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ours_sag_6.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&        
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/gt_cor_6.png}
            \caption{\hspace{4em}PSNR/SSIM}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/gt_sag_6.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}\\        
        
        9 & 
        
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ossart_cor_8_arrow.png}
            \caption{\hspace{4em}36.91/0.962}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ossart_sag_8.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/sup_cor_8.png}
            \caption{\hspace{4em}39.69/0.976}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/sup_sag_8_arrow.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ours_cor_8.png}
            \caption{\hspace{4em}\bf{41.16/0.980}}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/ours_sag_8.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}&        
        \begin{tabular}[b]{cc}
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/gt_cor_8.png}
            \caption{\hspace{4em}PSNR/SSIM}
            \end{subfigure} &
            \begin{subfigure}[b]{0.112\linewidth} \includegraphics[width=\textwidth,height=0.86\textwidth]{imgs/dvf_imgs/gt_sag_8.png}
            \caption{}
            \end{subfigure} 
        \end{tabular}\\     
        \hline
    \end{tabular}
    \caption{Visual comparisons of DVF-based reconstructions. Static structures as indicated by the orange arrows shift significantly in $\textrm{OSSART}^{\textrm{DVF}}$ due to badly estimated DVFs. Metrics are calculated volume-wise.}
    \label{tab:dvf_img}
    \vspace{-1.5em}
\end{figure*}

==> method.tex <==
\section{Method}

\begin{figure*}[!htb]
    \centering
      \includegraphics[width=1\textwidth]{imgs/REGAS_net.png}
    \caption{REGAS synthesizes unobserved views for phase $i$ based on observed views across all phases. It first takes the RPT transformed initial reconstructions $R^{\textrm{init}}_{i,a_k}$ and refines them through a 3D network $\mathcal{G}$. The resulting $R^{\textrm{ref}}_{i,a_k}$ forms views $P^{\textrm{ref}}_{i,a_k}$ and goes through a 2D network $\mathcal{F}$, yielding $P^{\textrm{out}}_{i,a_k}$. After training, $P^{\textrm{out}}_{i,a_k}$ are used to reconstruct $V^{\textrm{PS}}_{i}$. As a post-processing step, $V^{\textrm{PS}}_{i}$ can be used to estimate the between-phase DVFs $\mathcal{M}_{i\rightarrow j}$, which can be used to deform backprojections and allow multi-phase reconstruction based on just the observed views.}
    \label{fig:network}
    \vspace{-1.5em}
\end{figure*}
We define $P_{i,a_k}\in\mathbb{R}^{W\times H}$ as the acquired views of the $i^{\textrm{th}}$ phase $V_{i}$ along angle $a_k$, where $i\in\{1,2,...,N\}$ and $k\in\{1,2,...,K\}$. $N$ is the total number of phases that represents a complete respiratory cycle and $K$ is the total number of views acquired. Ideally, we acquire $K$ views for each phase $i$ to achieve high quality 3D reconstruction; in practice, we only acquire $K_i$ views for phase $i$, such that $K=\sum_{i}K_i$, i.e. a single 3D CBCT acquisition. Each observed view $P^{\textrm{obs}}_{\phi(a_k),a_k}$ over angle $a_k$ therefore corresponds to phase $\phi(a_k)$, where the correspondence $\phi(*)$ is measured or estimated. The goal of our proposed REGAS is to synthesize views based on $P^{\textrm{obs}}_{\phi(a_k),a_k}$ from a single CBCT acquisition, such that each phase has $K$ views for artifact reduced 4D CBCT reconstruction.


% \haofu{the previous sentences (to the beginning of this paragraph) do not seem to closely related to the context. Consider move them to section 3.2}
In the following sections, we first describe RPT, which addresses the heavy computational burden, propagates gradients between views and volumes, and enables distributed patch-based training for REGAS. We then describe the full REGAS pipeline for view synthesis. Finally, we describe how to use the REGAS reconstructions to find between-phase DVFs, which can be used for phase reconstructions where only real acquisitions $P^{\textrm{obs}}_{\phi(a_k),a_k}$ are used.


% Instead of addressing reconstruction directly in the CT domain, RGVS seeks to solve the problem by completing the projection data, i.e. such that $|a^{i}_{aug}| = K_{tot}, \forall i$ after augmentation. This is similar to the view synthesis task in nature image domain. Such a formulation allows us to use computationally intensive methods like deep learning to tackle the most direct measurements, and allow analytic 3D reconstruction, which is also computationally intensive, to happen as a post-process. 

% Many works have shown that 2D view synthesis requires a strong 3D grounding to be reliable[cite SinSyn, XraySyn]. As each phase already has several observed projections, the most intuitive approach is to do a partial 3D reconstruction and refine it through a 3D CNN, as constrained by  This presents a major challenge in computing resource, as 3D CNN has a cubic complexity and 


% We first describe our proposed Ray Path Transformation (RPT), which enables distributed patch training for a volume-projection hybrid training algorithm under a cone beam geometry. We then explain the full RGVS pipeline, which completes projection data for each phase for higher quality phase reconstruction. Finally we use these reconstructions to find between-phase DVFs, which allow us to reconstruct using only measured projections, thus allowing for maximum quality and reliability. (also explain why 3D to 2D is needed)

%This idea is similar to the dual-domain reconstruction popularly used in slice-wise CT reconstruction to reduce metal artifacts, where certain patterns are easier to be recovered from sinogram. Accurately estimating the missing projections can be formulated as a view synthesis problem, (add XraySyn in related work) where a strong knowledge of grounding in 3D is needed. As XraySyn has shown, such grounding is often computationally expensive in neural networks as dense volumetric representation. Therefore, we first describe our proposed Ray Path Transformation (RPT) module, which simultaneously serves as a differentiable forward projector and helps conserve memory.

\input{RPT}




% \subsection{Ray Path Transformation}

% RPT is proposed to address the memory bottleneck within REGAS, specifically the processing of high resolution volumetric CT in an end-to-end, 3D-to-2D CNN method. To achieve end-to-end learning, CT volumes cannot be broken down to patches as ray tracing requires full information during its traversal. The only solution without RPT is to downsample the CT volumes to compromise for GPU memory constraint, as shown in Fig. \ref{fig:RPT}. We also note that during CBCT acquisition, each view only observes a part of the volume. As such, a downsampled volume leads to significant loss in quality for each view, even though the entire volume is not needed for a particular view synthesis.


% Since every pixel on $P^{\textrm{obs}}_{i,a_k}\in\mathbb{R}^{W\times H}$ measures the projection of a ray from the light source, we consider representing the $P^{\textrm{obs}}_{i,a_k}$-observed CT volume as a series of rays. To this end, we define a ray-based representation of a CT volume $V_{\textrm{CT}}\in \mathbb{R}^{X\times Y\times Z}$ as $R\in \mathbb{R}^{W\times H\times S}$, where $S$ is the marching dimension of each ray, such that $P(w, h) = \sum_{s}R(w, h, s)$. RPT is thus defined as $\mathcal{T}(V, \psi):\mathbb{R}^{X\times Y\times Z} \to \mathbb{R}^{W\times H\times S}$ where $\psi$ includes projection parameters such as view angle $a_k$ and detector size $\{W, H\}$. As shown in Fig. , RPT records the values of rays $\bm{l}_{w,h}$ that traverse $V_{CT}$ at every marching step and organize them into a volume, which can be described as:
% \begin{align}\label{eqn: RPT}
% \begin{aligned}
%     R(w,h,s) = \mathcal{T}(V_{\textrm{CT}}, \psi) = V_{\textrm{CT}}(a^{-1}_k \bm{l}_{w,h}(s)),
% \end{aligned}
% \end{align}
% where view angle $a_k$ represents the homogeneous matrix that transforms coordinates in $V_{\textrm{CT}}$ to $\bm{l}_{w,h}$. 

% RPT has several distinct advantages: 1. it is memory-efficient in representing only the 3D context related to a particular view; 2. the transformed $R$ can be easily split and recombined over the $w-h$ plane while maintaining integrity to the forward projection process. This allows us to leverage the translational invariance of CNNs through patch learning, thus resolving the memory bottleneck in training 3D CNNs; 3. after transformation, forward projection is simplified to a summation operation along the ray marching dimension, eliminating the need for a specialized code for backpropogation; 4. by using the view-varying nature of the transformed volume, RPT serves as a form of data augmentation over the volumetric CT image. RPT is implemented through CUDA and is as fast as other GPU-implemented forward projection operations.


% To better illustrate the utility of RPT, an example is shown in Fig. 1. The acquired X-ray projections are typically of high resolution, therefore they requires a high resolution volume to capture the detail level during reconstruction. As synthesis on missing projections requires 3D context, $V^{\textrm{init}}_{i}$ is put into a CNN structure and thus memory constrained. Without RPT, we need to downsample $V^{\textrm{init}}_{i}$, which is the first degradation in quality. Furthermore, physically the detector only observes a part of the volume; as such heavy interpolations happen during forward projection, especially near the light source, hence a second degradation in quality. RPT cuts out the middle man, and directly yields the region of high resolution volume that the projection observes. Furthermore, $R$ can be separated to appropriate sizes, effectively removing memory limitation during training.


%In conception, the relationship between $R$ and $P$ is equivalent to $V$ and $P$ if parallel beam geometry is used for projection, as is done in X2CT-GAN; however, the equivalence is only true over two view angles. RPT is more generalized and can be used in real clinical reconstruction. RPT is implemented through CUDA. 

\subsection{REspiratory-GAted Synthesis (REGAS)}

To synthesize unobserved views, we would like to incorporate information from observed data. As such, we first obtain $V^{\textrm{init}}_{i}$ by performing algebraic reconstructions on $P^{\textrm{obs}}_{\phi(a_k),a_k}$, i.e. $V^{\textrm{init}}_{i} = \mathcal{H}(P^{\textrm{obs}}_{\phi(a_k),a_k})\hspace{0.3em} \forall a_k \hspace{0.3em} s.t. \hspace{0.3em} \phi(a_k)=i$, where $\mathcal{H}$ denotes methods like FBP or SART.
% \haofu{Two issues: 1) it seems that $P^{\textrm{obs}}_{\phi(a_k),a_k}$ means both a single view or a collection of all acquired views. needs separate notations for these two. 2) ``algebraic 3D reconstructions on $P^{\textrm{obs}}_{\phi(a_k),a_k}$" may be confusing (partially due to the first issue) for under-informed readers. need a clear description.}
Note that some $V^{\textrm{init}}_{i}$'s have higher quality than others, as phases have different durations and number of observed views. 

% As shown in Fig. \ref{fig:network}, REGAS is an end-to-end network that contains a 3D and a 2D CNN, which provides the context and freedom needed for synthesizing missing views. 

REGAS consists of a 3D CNN and a 2D CNN, which processes $V^{\textrm{init}}_{i}$ and the subsequent projected views over various view angles. In the first stage, the 3D CNN $\mathcal{G}$ has a 3D-UNet \cite{DBLP:conf/miccai/CicekALBR16} like architecture and uses all the reconstructed phases $V^{\textrm{init}}_{i}$ as inputs. This allows for structural information to be shared across phases, \textit{e.g.,} phase-invariant features such as the static bone structure can be shared from higher quality phases to lower quality phases. Due to the high resolution of $V^{\textrm{init}}_{i}$, training on a sufficiently deep $\mathcal{G}$ is only feasible by first transforming $V^{\textrm{init}}_{i}$ to $R^{\textrm{init}}_{i,a_k}$ through RPT and decomposing them to patches. The forward process of $\mathcal{G}$ can be described as:
\begin{align}\label{eqn: 3DCNN}
\begin{aligned}
    \{R^{\textrm{ref}}_{1,a_k},R^{\textrm{ref}}_{2,a_k},...,R^{\textrm{ref}}_{N,a_k}\}=\mathcal{G}(R^{\textrm{init}}_{\forall i,a_k}) + R^{\textrm{init}}_{\forall i,a_k}\\
    R^{\textrm{init}}_{\forall i,a_k} = R^{\textrm{init}}_{1,a_k} \oplus R^{\textrm{init}}_{2,a_k}\oplus...\oplus R^{\textrm{init}}_{N,a_k},
\end{aligned}
\end{align}
where $\oplus$ concatenates $R^{\textrm{init}}_{i,a_k}$ over the channel dimension. We can then obtain views through forward projection, i.e. $P^{\textrm{ref}}_{i,a_k} = \sum_{s}R^{\textrm{ref}}_{i,a_k}$.

The second view-refining stage consists of an RDN-based \cite{DBLP:conf/cvpr/ZhangTKZ018} 2D CNN $\mathcal{F}$, which individually processes views from each phase and can be described as: \begin{align}\label{eqn: 2DCNN}
\begin{aligned}
    P^{\textrm{out}}_{i,a_k}=\mathcal{F}(P^{\textrm{ref}}_{i,a_k})+P^{\textrm{ref}}_{i,a_k}.
\end{aligned}
\end{align} 
As described, residual learning is used in Eq. (\ref{eqn: 3DCNN}) and Eq. (\ref{eqn: 2DCNN}) to promote faster convergence.

Due to the limited data availability for supervision and the changing imaging condition, we seek to train $\mathcal{G}$ and $\mathcal{F}$ by exploring the rich information within observed views. For every $a_k$, we have one observed view, which can be used as an $\mathcal{L}_1$ reconstruction constraint with its synthesis: 
\begin{align}\label{eqn: recon_loss}
\mathcal{L}_{\textrm{rec}}=\lVert P^{\textrm{out}}_{\phi(a_k),a_k} - P^{\textrm{obs}}_{\phi(a_k),a_k}\rVert_1.
\end{align}
While we do not have observed views for other phases, we note that these phases are observed at only slightly rotated angles, if the total number of acquisitions $K$ is sufficiently dense, which is true in real applications \cite{shieh2019spare}. We therefore use a patch-wise GAN loss to constrain training on unobserved views, described as:
\begin{align}\label{eqn: 2DCNN_GAN}
\begin{aligned}
\mathcal{L}^{\mathcal{D}}_{\textrm{GAN}}(P^{\textrm{out}}_{i,a_k}, P^{\textrm{obs}}_{i,nbr(i,a_k)})&=\\
\mathbb{E}(\mathcal{D}(P^{\textrm{obs}}_{i,nbr(i,a_k)}-1)^2)) &+
\mathbb{E}(\mathcal{D}(P^{\textrm{out}}_{i,a_k}-0)^2)\\
\mathcal{L}^{\mathcal{G}}_{\textrm{GAN}}(P^{\textrm{out}}_{i,a_k})&=\mathbb{E}(\mathcal{D}(P^{\textrm{out}}_{i,a_k}-1)^2),
\end{aligned}
\end{align} 
where $nbr(i,a_k)$ yields the closest neighboring view angle from $a_k$ that observes phase $i$. %We find that a GAN formulation can leverage the strong statistical similarity between $P^{\textrm{obs}}_{i,nbr(i,a_k)}$ and $P^{\textrm{obs}}_{i,a_k}$, despite their pixel-wise difference.

Additionally, we propose a self-supervised loss at the volumetric level. We denote $V^{\textrm{ma}}$ as the motion-affected CT reconstruction by using views of all phases. $V^{\textrm{ma}}$ is blurry over regions that are moving; however, it is of high quality over static regions. As $\mathcal{G}$ generates $R^{\textrm{ref}}_{i,a}$ of all phases $i$, the voxel-wise average of these phase reconstructions similarly follows this observation; therefore, we define a motion averaging loss:
\begin{align}\label{eqn:3D_loss}
\mathcal{L}_{\textrm{MA}}=\lVert \frac{1}{N}\sum_{i}R^{\textrm{ref}}_{i,a_k} - R^{\textrm{ma}}_{a_k}\rVert_1, 
\end{align}
where $R^{\textrm{ma}}_{a_k}$ is transformed through RPT from $V^{\textrm{ma}}$ over view angle $a_k$. We find that while $\mathcal{L}_{\textrm{MA}}$ is an inexact loss due to the different reconstruction procedures, it is useful in stabilizing the network and suppressing sparse-view artifacts in $R^{\textrm{init}}_{i,a}$. The overall loss for training the full REGAS is therefore:
\begin{align}\label{eqn:overall_loss}
\mathcal{L}_{\textrm{all}}=\lambda_{\textrm{MA}}\mathcal{L}_{\textrm{MA}} + \lambda_{\textrm{rec}}\mathcal{L}_{\textrm{rec}} + \lambda_{\textrm{GAN}}\mathcal{L}_{\textrm{GAN}}, 
\end{align}
where $\lambda_{\textrm{MA}}$, $\lambda_{\textrm{rec}}$, and  $\lambda_{\textrm{GAN}}$ are weights for their respective loss, empirically chosen as 1, 0.1, and 0.05, respectively.

% Based on RPT, we describe our proposed RGVS network at synthesizing unobserved projections of a given phase. 

% As shown in Fig. 2, RGVS is an end-to-end trainable, 3D-to-2D CNN network. First, to eliminate noise and promote information sharing between initially reconstructed phases, we propose a self-supervised 3D loss called motion average loss. The idea of MAL is that the average of all phases should be similar to a reconstruction using all observed projections. 


% The high resolution volumes $V^{\textrm{init}}_{i}$ are first transformed through RPT to obtain $R^{\textrm{init}}_{i,a}$ along view angle $a$. All phases of $R^{\textrm{init}}_{i,a}$ are concatenated in the channel dimension as the input to a 3D CNN $\mathcal{G}$. Mathematically this is expressed as:
% \begin{align}\label{eqn: 3DCNN}
% \begin{aligned}
%     \{R^{\textrm{ref}}_{1,a},R^{\textrm{ref}}_{2,a},...,R^{\textrm{ref}}_{N,a}\}=\mathcal{G}(R^{\textrm{init}}_{1,a} \oplus R^{\textrm{init}}_{2,a}\oplus...\oplus R^{\textrm{init}}_{N,a}).
% \end{aligned}
% \end{align}

% This provides a signal to maintain a degree of 3D consistency and prevent collapse of the overall system - as without it the network can degrade to using the phase with the highest quality for 2D stage. Specifically the 3DCNN network can dynamically determine the proper weights voxel-wise that help establish the relationship. 
% The overall results 



\input{tables/metrics}
\subsection{Between-phase DVF Estimation}\label{sec:dvf}
After REGAS is trained to convergence, we can complete the missing views by performing inference on $V^{\textrm{init}}_{i}$ over all $a_k$. After completion, $P^{\textrm{out}}_{i,a_k}$ and $P^{\textrm{obs}}_{\phi(a_k),a_k}$ are used to reconstruct the final phases, denoted as $V^{\textrm{VS}}_{i}$. 

To further improve quality, 
%Due to the high quality of $V^{\textrm{VS}}_{i}$, 
we incorporate $V^{\textrm{VS}}_{i}$ into a \textit{DVF-based post-processing} step. To do so, we find the deformation field $\mathcal{M}_{i\rightarrow j}$ between each phase pair $<V^{\textrm{VS}}_{i},V^{\textrm{VS}}_{j}>$, using a well-performing 3D registration methods, e.g. \cite{AVANTS200826,DBLP:journals/tmi/BalakrishnanZSG19}. After obtaining DVFs, we apply a deformed FBP to reconstruct phases based on only $P^{\textrm{obs}}_{\phi(a_k),a_k}$, as shown in Fig \ref{fig:network}. Specifically, during backprojection where the filtered pixels on $P^{\textrm{obs}}_{\phi(a_k),a_k}$ are traced back to the light source, we deform ray paths according to $\mathcal{M}_{\phi(a_k)\rightarrow j}$, where $j$ is the intended phase for reconstruction. Deformed rays from all $a_k$'s are summed over the common volumetric space, yielding $V^{\textrm{DVF}}_{j}$. 

Since $V^{\textrm{DVF}}_{j}$ is reconstructed with observed data, it contains much less artifacts induced by the sparse-view condition; however, the accuracy of $V^{\textrm{DVF}}_{j}$ depends on the assumptions within the DVF reconstruction formulation, \textit{i.e.,} breathing motion is accurately modeled by DVFs. We discuss in Section \ref{sec:dvf_exp} the advantages and disadvantages of DVF-based reconstruction.

% We can then use $\mathcal{M}_{pha(a_k)\rightarrow j}$ to warp the backprojection trajectory of $P^{\textrm{obs}}_{pha(a_k),a_k}$ to all other phases $j$, thus achieve reconstructing all phases with only observed data.





==> tables/metrics.tex <==
\begin{table*}[!htb]
\setlength{\tabcolsep}{1pt}
\centering 
\begin{tabular}{| l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
 Phase & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9& 10 &Average\\
\hline
OSSART 
& 35.1/.942
& 34.4/.933
& 31.7/.870
& 34.3/.927 
& 34.5/.934
& 32.1/.883 
& 31.4/.864 
& 30.4/.835 
& 32.0/.879 
& 31.8/.872
& 32.8/.894\\

% $\textrm{UNet}^{small}_{sup}$ 
% & 34.9/.945
% & 34.7/.945
% & 34.0/.835
% & 34.8/.945
% & 34.8/.946
% & 34.4/.940
% & 33.8/.933
% & 33.4/.928
% & 34.2/.936
% & 34.2/.938
% \\

$\textrm{UNet}_{\textrm{sup}}$ 
& 36.7/.959
& 36.6/.959
& 35.2/.946
& 36.6/.958
& 36.7/.960
& 35.7/.952
& 34.8/.942
& 34.1/.935
& 35.4/.944
& 35.5/.949
& 35.7/.950
\\

$\textrm{REGAS}_{\textrm{2D}}$ 
&  37.6/.966
&  36.7/.958
&  33.4/.909
&  36.7/.957
&  36.9/.960
&  34.2/.922
&  33.0/.899  
&  31.2/.864
&  33.7/.913
&  33.8/.914
&  34.7/.926
\\
$\textrm{REGAS}_{\textrm{noRPT}}$
&  37.1/.965
&  36.5/.959
&  34.1/.923
&  36.4/.956
&  36.7/.960
&  34.8/.936  
&  33.8/.915
&  32.5/.894
&  34.5/.929
&  34.2/.926
&  35.1/.936
\\
$\textrm{REGAS}_{\textrm{noMA}}$ 
&  37.5/.967
&  37.2/.965
&  35.7/.946
&  37.1/.964
&  37.3/.964            
&  36.1/.952
&  35.5/.944
&  34.3/.923
&  35.8/.950
&  35.8/.948
&  36.2/.952
\\
$\textrm{REGAS}$ 
&  \bf{39.1/.977}
&  \bf{38.7/.974}
&  \bf{37.6/.964}
&  \bf{38.5/.973}
&  \bf{38.7/.974}
&  \bf{37.8/.966}      
&  \bf{36.9/.957}
&  \bf{35.5/.938}
&  \bf{37.4/.964}
&  \bf{37.4/.964}
&  \bf{37.8/.965}
\\
\hline
\hline
% FBP & N/A & &&&&&&&&\\
$\textrm{OSSART}^{\textrm{DVF}}$ & 39.0/.974 
& 39.0/.973
& 37.4/.969
& 39.1/.973
& 39.1/.971
& 37.5/.968
& 35.9/.960
& 34.3/.943
& 37.3/.965
& 37.4/.967
& 37.6/.966
\\
$\textrm{UNet}^{\textrm{DVF}}_{\textrm{sup}}$ 
& 40.2/.980
& 40.8/.980
& 40.1/.982
& 40.3/.978
& 39.5/.975
& 38.3/.977
& 37.6/.975
& 37.3/.971
& 39.9/.978
& 39.7/.979
& 39.4/.978
\\
$\textrm{REGAS}^{\textrm{DVF}}$ 
& \bf{41.8/.984} 
& \bf{42.3/.984}
&\bf{42.6/.988}
&\bf{41.8/.982}
&\bf{41.6/.980}
&\bf{41.3/.985}
&\bf{40.9/.984}
&\bf{40.1/.981}
&\bf{41.3/.982}
&\bf{41.8/.985}
&\bf{41.6/.983}
\\
\hline
\end{tabular}
\caption{Quantitative evaluation of 4D RG-CBCT reconstruction on 4D Lung~\protect\cite{2017A} in terms of PSNR and SSIM. The best results are in {\bf bold} in both algebraic and DVF-based reconstructions. Phases that have more observed views have higher PSNRs in their OSSART reconstructions.}
\vspace{-1em}
% , and the second best results are \underline{underlined}.}
\label{tab:sota_table}
\end{table*}

==> tables/temp.tex <==
\begin{table*}[!htb]
\setlength{\tabcolsep}{1pt}
\centering 
\begin{tabular}{|c|ccc|ccc|ccc|ccc|}
\hline
 Method & \multicolumn{3}{c|}{DiNTS} & \multicolumn{3}{c|}{Meta-Oneshot} & \multicolumn{3}{c|}{DiNTS} & \multicolumn{3}{c|}{Meta-Oneshot} \\
\hline
Memory
& \multicolumn{3}{c|}{5067MiB}
& \multicolumn{3}{c|}{5358MiB}
& \multicolumn{3}{c|}{8802MiB}
& \multicolumn{3}{c|}{7168MiB} \\
\hline

& DSC1
& DSC2
& Avg.
& DSC1
& DSC2
& Avg.
& DSC1
& DSC2
& Avg.
& DSC1
& DSC2
& Avg.
\\
\hline
Pancreas 
& 77.41
& 47.51
& 62.46
& \bf{78.90}
& \bf{50.22}
& \bf{64.56}
& 80.06
& 52.53
& 66.29
& \bf{80.10}
& \bf{53.47}
& \bf{66.79}
\\
\hline
Liver
& 93.42
& 50.26
& 71.84
& \bf{93.95}
& \bf{56.97}
& \bf{75.46}
& \bf{94.32}
& 57.64
& 75.98
& 94.21
& \bf{57.77}
& \bf{75.99}
\\
\hline
\end{tabular}
\caption{Compared to DiNTS, our proposed Meta-Oneshot finds better structures. Specifically, our small compute model performs much better than DiNTS', and our large compute model is competitive with DiNTS' with less memory usage.}
\vspace{-1em}
% , and the second best results are \underline{underlined}.}
\label{tab:sota_table}
\end{table*}

==> tables/temp_multi.tex <==
\begin{table*}[!htb]
\setlength{\tabcolsep}{1pt}
\centering 
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
 Method & \multicolumn{3}{c|}{DiNTS} & \multicolumn{3}{c|}{Meta-Oneshot} & \multicolumn{3}{c|}{MT-Meta-Oneshot} \\
\hline
Memory
& \multicolumn{3}{c|}{8802MiB}
& \multicolumn{3}{c|}{7168MiB}
& \multicolumn{3}{c|}{7000MiB} \\
\hline

& DSC1
& DSC2
& Avg.
& DSC1
& DSC2
& Avg.
& DSC1
& DSC2
& Avg.
\\
\hline
Pancreas 
& 80.06
& 52.53
& 66.29
& \bf{80.10}
& 53.47
& \bf{66.79}
& 79.85
& \bf{53.65}
& 66.75
\\
\hline
Liver
& 94.32
& 57.64
& 75.98
& 94.21
& 57.77
& 75.99
& \bf{94.39}
& \bf{58.84}
& \bf{76.62}
\\
\hline
Hepatic Vessel
& 60.85
& 66.96
& 63.91
& 60.80
& 66.72
& 63.76
& \bf{61.59}
& \bf{69.93}
& \bf{65.76}
\\
\hline
\end{tabular}
\caption{Our Multi-Task (MT) Meta-Oneshot model provides additional improvements by using a single model for a combined dataset of three different tasks. Particularly, by sharing weights for three tasks, we reduce training time by $50\%$ compared to individual training; furthermore, we observe performance improvements on the Liver and Hepatic Vessel datasets, and competitive performance over the Pancreas dataset.}
\vspace{-1em}
% , and the second best results are \underline{underlined}.}
\label{tab:sota_table}
\end{table*}
